The Dawn of Disaggregation and the Coherence Conundrum: A Call for Federated Coherence

Disaggregated memory is an upcoming data center technology that will allow nodes (servers) to share data efficiently. Sharing data creates a debate on the level of cache coherence the system should provide. While current proposals aim to provide coherence for all or parts of the disaggregated memory, we argue that this approach is problematic, because of scalability limitations and hardware complexity. Instead, we propose and formally define federated coherence, a model that provides coherence only within nodes, not across nodes. Federated coherence can use current intra-node coherence provided by processors without requiring expensive mechanisms for inter-node coherence. Developers can use federated coherence with a few simple programming paradigms and a synchronization library. We sketch some potential applications.

==> Texts/Background.tex <==
\section{Background }
\label{sec:background}

\subsection{Shared Disaggregated Memory}
In this paper, we focus on distributed systems that use shared disaggregated memory\footnote{In this paper,
  the term (shared) disaggregated memory refers to
  memory addressable by 
  load and store instructions, as opposed to mechanisms such as
  RDMA or page faults (which are less concerned
  about cache coherence).} for communication. There is a longstanding debate about whether message passing or shared memory is the best way to build scalable systems. We do not take a position on this debate; instead, we note that existing hardware has made it feasible to build shared memory systems using off-the shelf parts. At the same time, the increasing memory demands of modern workloads, and a slowdown in the
  improvement of local memory capacity has led to increased adoption of disaggregated memory systems. These systems allow multiple servers to combine their compute power to
  process data placed on large pools of shared memory, and could 
 provide the computational capacity of an expensive scale-up supercomputer~\cite{nvidia_dgx_gh200} using commodity hardware.
While early disaggregated memory deployments have 8--16 sockets~\cite{pond}, we envision future rack scale
system with 20--80 servers using CXL v3 switches~\cite{cxl}.
  
Disaggregated memory is not a new concept~\cite{LCMRRW2009}
  but recently, several technologies have emerged
  to support it, including CC\-IX~\cite{ccix}, Gen-Z~\cite{genz},
  OpenCAPI~\cite{opencapi}, and more recently CXL~\cite{cxl},
  which has become an industry standard with broad
  support from hardware vendors.
Conventional wisdom says that shared memory should be cache coherent~\cite{MHS2012},
and the latest CXL v3 specification supports it.
  
\subsection{Modern Cache Coherence struggle with many core and heterogeneous compute}
The challenges of cache coherence have become increasingly complex with the rise of many-core processors and heterogeneous architectures. Modern systems provide valuable insights into the evolving strategies for managing coherence in complex environments, offering precedents that are highly relevant to the emerging landscape of disaggregated memory.

In many-core architectures, large multi-core chips are often logically organized into clusters or tiles of cores to improve performance and scalability.
This structure naturally lends itself to a hierarchical approach to coherence. 
Within a cluster, a traditional full coherence protocol (like MESI or MOESI) is typically employed to maintain consistency between the caches of cores that share a lower-level cache (e.g., L2). 
This ensures high performance for tightly-coupled workloads within the cluster.
However, scaling these full coherence protocols to a large number of cores becomes increasingly challenging due to increased communication overheads.
Coherence between different clusters however, is often managed through different, and potentially more relaxed, mechanisms.
Directory-based protocols are common, but they may offer weaker consistency guarantees or incur higher latency compared to intra-cluster coherence, reflecting the understanding that communication patterns are frequently localized. 
In Non-Uniform Memory Access (NUMA) architectures, where memory access times vary depending on the memory location relative to the processor, the hierarchical nature of coherence is even more pronounced.
Coherence protocols are typically layered, reflecting the varying access latencies: cores sharing an L3 cache within a NUMA node maintain the strictest coherence, followed by coherence within the same physical socket, and finally, across the entire system. 
This mirrors the increasing communication costs as data is accessed further away. 
This hierarchical approach limits the scope of strict coherence, which is necessary for scaling to a large number of cores, a similar problem that disaggregated memory faces.

ARM's heterogeneous architectures, such as systems combining high-performance 
    Cortex-A cores with real-time Cortex-R cores, provide compelling examples of partial or asymmetric coherence. 
In these systems, coherence might be enabled only between specific sets of cores 
    (e.g., among Cortex-A cores within a cluster), while others (e.g., Cortex-R cores) are left non-coherent. 
Further, ARM's AMBA Coherent Hub Interface (CHI) allows for selective coherence by enabling certain regions of memory or specific transactions to be marked as "non-coherent".
This can be achieved, for example, through attributes in the memory management unit (MMU) or by using specific transaction types that bypass coherence mechanisms. 
These examples from ARM highlight that for performance and efficiency, full coherence is not always the optimal solution and that software needs to be aware of the coherence domain.

Systems that integrate CPUs with GPUs or other specialized accelerators further demonstrate the move away from strict, universal coherence. 
Maintaining full cache coherence across these disparate processing units is often deemed impractical or too costly in terms of performance overhead. 
Instead, data consistency is often managed through explicit synchronization primitives, software-managed caches, or specialized memory regions with relaxed consistency models.
Technologies like RDMA, commonly used for remote memory access, also typically bypass cache coherence mechanisms, relying on explicit software management for data consistency. 
In many cases, the pragmatic choice is to not enforce full coherence, accepting the increased responsibility on the programmer to manage data consistency in exchange for improved performance.

\subsection{Lessons from today to tomorrow}
The evolution of coherence strategies in modern systems offers several crucial takeaways that are directly applicable to the challenges of disaggregated memory. 
First, the hierarchical approach to coherence within a single node, particularly in NUMA systems, demonstrates a clear move towards more nuanced and localized coherence strategies. 
This is driven by the need to manage the increasing complexity and communication costs inherent in large multi-core architectures—challenges that are significantly amplified in disaggregated memory systems.  
Second, the deliberate choice to forgo full coherence in heterogeneous systems, especially with accelerators, highlights the performance trade-offs (or increased programmer burden) associated with maintaining strict consistency across diverse processing units. 
It demonstrates that alternative, less strict coherence models are not only feasible but often preferable.
In disaggregated memory, the diversity of access patterns and the potential for large numbers of connected nodes further strengthen this argument. 
Third, if managing coherence is a significant challenge within a single node with a logarithmic increase in the number of cores, the introduction of disaggregated memory, with its potential for a log-log scale increase in potentially coherent entities, necessitates a serious and open discussion about alternative coherence models.
The sheer scale and distributed nature of disaggregated memory make it highly unlikely that full, hardware-managed coherence will be the most efficient or scalable solution.
Furthermore, the experience from heterogeneous systems suggests that software can take advantage of the relaxed coherence to improve performance. 
In conclusion, it is not only imperative that we engage in a discussion about the appropriate level of coherence for disaggregated memory, but also important to realize that it is possible to deviate from the traditional binary choice of full or no coherence. 
The experience gained from many-core and heterogeneous systems strongly suggests that exploring alternative coherence models, such as our proposed Federated Coherence, is essential to unlocking the full potential of disaggregated memory.



\subsection{Cache Coherence and Its Cost}
\label{sec:costcoherence}

Hardware-based cache coherence is prevalent in
  modern 
  multi-core processors.
Typically, each core has individual small caches (\eg{} L1 and L2), and the cores within a processor package share a larger cache (\eg{} L3).
As many cores may access the same memory locations, a location can be simultaneously present in multiple caches.
Cache coherence ensures that
  different cores are provided a consistent view of a
  cache line.
For example, if a cache line present in multiple caches gets modified by a core, cache coherence ensures that the cache lines are either invalidated or updated.

Cache coherence is implemented through a protocol
that involves CPUs and caches.
This protocol scales poorly because it must
  coordinate the execution of operations across all participant caches, creating a communication bottleneck.
For example, in the MESI coherence protocol~\cite{mesi}, each cache
  line can be in one of four states (Modified, Exclusive, Shared, Invalid), and the caches coordinate to ensure that lines for the same location in different caches are in compatible states.
Keeping track of cache line states means that caches need to snoop on the bus, creating a point of contention that limits scalability.
Alternatively, systems with a large number of cores, including
  CXL-based disaggregated memory, use directory-based coherence protocols,
  which scale better
  but add complexity and latency to accesses, and their scalability still falters when a cache line is widely shared.

\begin{figure}[]
    \centering
    \includegraphics[width=0.9\columnwidth,trim={20pt 10pt 20pt 10pt},clip]{figures/AMD Topology.pdf}
    \caption{Evaluation platform. A two-socket AMD EPYC 7754 server,
    with 128 cores per socket. Each socket has 16 core
    complexes with 8 cores each. A core complex corresponds to
    a \emph{soft-NUMA domain}: communication latency is smallest between CPUs in the same complex (same soft-NUMA domain), then within the same socket (same NUMA domain), then across sockets (different NUMA domains), as shown by the latency numbers in blue.
    The server runs RedHat Enterprise Linux 9 with the 5.14 kernel.
    }
    \label{fig:hardware}
\end{figure}

\begin{figure*}[t]
  \centering
  \begin{subfigure}[t]{0.32\textwidth} % Adjust width for 3 graphs
    \includegraphics[width=\textwidth]{figures/extrapolate.pdf}
    \vspace{-7mm}
    \caption{}
    \label{fig:many_core}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figures/differential.pdf}
    \vspace{-7mm}
    \caption{}
    \label{fig:derivative}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figures/softnuma.pdf}
    \vspace{-7mm}
    \caption{}
             %Placing threads across multiple soft NUMA nodes exacerbates the performance degradation, highlighting the impact of physical core location and cache coherence overhead.}
    \label{fig:softnuma}
  \end{subfigure}
  \caption{(a) Overhead of cache coherence as we vary the number of cores. 
  (b) Derivatives of overhead in~\cref{fig:many_core}.
  (c) Overhead of cache cache coherence as we vary the number of soft NUMA domains.}
  
  \label{fig:allgraphs}
\end{figure*}


In the remainder of this subsection, we present experiments conducted to understand the cost of cache coherence using the hardware in \cref{fig:hardware}. As the figure shows, the communication between cores exhibits different latencies depending on whether the cores are in the same soft-NUMA domain, the same NUMA domain, or different NUMA domains.
This setup allows us to study the effect of communication latency on coherence overhead.

In the first experiment, we compare two scenarios.
In scenario 1, a number of threads run a loop that atomically increments a single common global variable, thereby producing significant coherence traffic.
Each thread is pinned to a fixed and dedicated set of cores.
Scenario 2 represents a non-cache coherent system.
Since our server is cache coherent, we mimic the behavior of incoherence by having each thread atomically increment a different local variable.
%rather than a common variable.
In both scenarios, we measure the rate of increment operations.
We calculate the \emph{coherence overhead} as the
  ratio between the non-cache coherent rate to
  the cache coherent rate, which represents the multiplicative slowdown
  caused by coherence.

The 'Empirical Single Node' line in \cref{fig:many_core} plots the measured coherence overhead as the number of cores increases.
The overhead increases nearly linearly with the number of cores, reaching 244 at 256 cores.
To further understand these results,
\cref{fig:derivative} shows the slope (derivative) of the
  coherence overhead curve in \cref{fig:many_core}, smoothed out by a Savitzky-Golay filter~\cite{filter}.
For the first 128 cores, the slope
  is smaller (${\approx}0.9$) as these cores
  are within the same NUMA domain.
The slope then increases to ${\approx}1.2$, corresponding
  to a higher overhead per additional core.
This increase happens because after 128 cores, we allocate
  new cores from the second NUMA domain, so the
  coherence protocol experiences higher
  communication latency, increasing the
  coherence overhead.

\if0
More precisely, the increase in the overhead is
  ${\approx}0.66$, ${\approx}2.81$, or ${\approx}5.0$ whenever we add
  a core in the same soft NUMA domain,
  a new soft NUMA domain, or a new NUMA domain,
  respectively.
These proportions $0.66 : 2.81 : 5.0$ closely track the
  proportions $25.8\t{ns} : 106.6\t{ns} : 184.9$\t{ns} of the
  communication latencies within a soft NUMA domain,
  across soft NUMA domains, and across NUMA domains
  in~\cref{fig:hardware}.
\fi

We next study the effect of communication latency on
  coherence overhead using the soft-NUMA properties of our platform.
From~\cref{fig:hardware}, the latency between
  two cores in the same soft-NUMA domain
  is smaller than across domains.
So we repeat the previous experiment with only 8 cores, but we vary the 
   number of soft-NUMA domains (within a socket)
   from which these cores are chosen.
As shown by \cref{fig:softnuma}, performance declines as we add more soft-NUMA domains.
When all threads are in the same soft NUMA domain, the
  coherence overhead is 4.3.
Crossing soft-NUMA boundaries increases the overhead to 7.3 with 2 soft-NUMA domains, peaking at 11 when using 8 soft-NUMA domains (\ie{} one core from each).
If we place threads across NUMA domains (not shown) rather than
  soft-NUMA domains, the coherence overhead is 13.5. 
Overall, we see that communication latency significantly affects 
  coherence overheads.

Hardware with shared disaggregated memory
is not yet commercially
available, so we estimate its coherence overhead as
 follows.
We consider three values for the communication
  between nodes using disaggregated memory:
  200, 400, or 800ns.
This corresponds to a best-case and worst-case
  estimate of disaggregated memory performance
  reported in a recent study~\cite{pond}.
To find the coherence overhead for these
  latencies, we extrapolate our empirical
  measurements of overhead for a single node
  as a function of the communication latency
  incurred for that node both
  within and across NUMA domains.
Through interpolation, we find a
  near linear relation between the
  derivative of the coherence overhead and
  the communication latency\footnote{Specifically,
   the slope of the graph from cores 1 to 128 (within a NUMA domain) is 0.87, while the slope from cores 129 to 256 (across NUMA) is 1.19.
   The proportion 0:87 : 1.19
   nearly matches the proportion 184.9ns : 106.6ns of the communication
   latency across and within NUMA domains 
   in~\cref{fig:hardware}.}.
Thus, for a communication latency of 200, 400, or 800ns
  under disaggregated memory, the
  derivative of the coherence overhead should be
  2.2, 4.5, or 8.9, respectively.
This estimate is shown as the Est Multi Node lines in
  \cref{fig:many_core}.
We see that cache coherence
  significantly  affects performance: with an 800ns
  latency, the coherence overhead exceeds
  1000 with 384 cores.

These experiments illustrate why cache coherence scalability is problematic for disaggregated memory. Two factors combine to cause costs to balloon:
the high number of cores, which increases coherence overheads linearly, and the larger communication latency, which proportionally increases its derivative.

==> Texts/Sec6_Discussion.tex <==
\section{Discussion}
\label{sec:discussion}
\notejae{1. do we need to pay the cost of coherence in disaggregation.(cc makes programming easier but is it worth dropping the easness of programmability) 
2. Are data structures sufficient to program incoherent memory?
3. Assume data structure (or other programming model) are sufficient, how can we realize this?
\textbf{Useful nightmare
}
}

==> Texts/old/Sec1_Introduction1.tex <==
\section{Introduction}
\label{sec:intro}

Physically disaggregated memory is a recent trend in data center design, where additional memory is made available to servers, decoupled from server enclosures, and placed in a memory blade that is connected by a fabric so that it can be accessed by multiple servers.
This architectural shift offers compelling advantages, including enhanced memory capacity and bandwidth as well as improved server resource utilization~\cite{das2023introduction,legoos,aguilera2023memory,cfm}.

More recent byte-addressable, shared instantiations of disaggregated memory add additional capability as an efficient data-sharing mechanism between servers.
By allowing hosts to directly share memory instead of exchanging data via the network, shared disaggregated memory can bypass network overheads, such as serialization and memory duplication, and lead to improved performance, particularly for modern distributed workloads that must collaboratively process increasing amounts of in-memory data~\cite{stephanie_ownership, exoshuffle, ramcloud, spark, rdds, graphx}.

In traditional single-server programming, concurrent shar\-ed memory processing is simplified with hardware-managed cache coherence.
These protocols support familiar primitives, such as atomics, locks, and critical sections, that help coordinate thread execution across different CPU cores.
%and the use of atomics and locks which can be used to coordinate threads run on different CPU cores, to implement critical sections, etc.
Proposals for shared-memory disaggregation---such as those built on Compute eXpress Link (CXL)---aim to allow a similar coherence model by using derivatives of well-known protocols like MESI.
While retaining coherence for disaggregated memory would allow programmers to use familiar abstractions, it suffers from two fundamental limitations.

\heading{Scalability.}
At a basic level, a coherence protocol involves coordination that is known to struggle with scaling to a large number of participants. 
%Despite its utility, cache coherence comes at a high price:
%  it requires an expensive coherence
%  protocol interposed on memory accesses
%  to ensure that caches 
%  do not lose updates or serve
%  stale data (\S\ref{sec:costcoherence}).
While the costs of cache coherence have been extensively debated in the context of multicore processors~\cite{MHS2012,scaleNUMA}, we note that hardware-based cache coherence will be significantly \textit{more} expensive for disaggregated memory compared to server-local implementations.

The reasons are twofold.
First, in disaggregated memory, many benefits only arise with a sufficiently large number of participant CPUs.
Second, the coherence protocol will experience a larger communication latency as components reside in different hosts.
For example, with CXL disaggregated memory, modifying memory cached in another node takes at least two remote round trips:
one to contact the \emph{home agent} of the cache line in disaggregated memory (essentially a directory), and another for the home agent to ask the other node to invalidate the cache line.
Additional communication is required if the remote cache line is dirty.


\heading{High resource requirements.}
Simultaneously, hardware-based cache coherence requires either a sufficiently large directory or snoop filter near the CXL switch or a broadcast-based invalidation approach.
Both options impose a significant burden on hardware complexity or communication bandwidth, especially as the system grows.

\noheading
Thus, a critical question arises: how should industry and the research community enable such disaggregated memory sharing across hosts?
Besides cache coherent shared memory regions, the CXL specification allows memory to be marked incoherent, which would scale well and reduce hardware complexity.
However, there is relatively limited prior experience integrating incoherent shared memory into modern distributed systems \noteamaro{''(an exception is Cosh~\cite{cosh} which we discuss in \S\ref{subsec:unscalable})''?}.
For example, fully incoherent memory prevents multiple threads from coordinating via memory, and they would instead need to rely on message passing, which significantly increases overheads.
Although some recent research proposals suggest splitting available regions into small coherent regions for coordination and larger incoherent regions for data~\cite{pasha, danielberger}, the coherent regions still leave the fundamental concerns in place.

%A critical question remains largely unsettled: 
%what level of cache coherence is truly necessary and optimal for this new paradigm?
%The debate surrounding coherence models is not new;
%it has long been an implicit discussion within the hardware community,
%particularly in the context of many-core architectures and heterogeneous systems. 
%Solutions ranging from full hardware-managed cache coherence, 
%    similar to that found in traditional SMP systems,
%    to directory-based approaches, and even software-managed coherence have all been explored,
%    each with its own set of trade-offs in terms of performance, complexity, and programmability.
%However, the scale and dynamic nature of disaggregated memory introduce new dimensions to this debate. 

%Today the choice is binary for hardware vendors:
%    either they provide full hardware-managed cache coherence or they offer no coherence guarantees at all.
%This is because the vast majority of existing software fundamentally 
%    relies on the assumption of full coherence, and there has been, as of yet,
%    no significant dialogue within the software community to explore or establish alternative models.
%This "all or nothing" situation presents a significant barrier,
%    potentially forcing hardware vendors into overly complex designs and ultimately 
%    hindering the exploration of more efficient and scalable coherence solutions specifically
%    tailored for the unique demands of the disaggregated era.
%Without a concerted effort to define and adopt new programming models that can accommodate
%    relaxed or partial coherence, software will remain tethered to the familiar,
%    albeit potentially limiting, expectation of full hardware coherence.

To address this conundrum, we propose a distributed cache coherence model called \emph{\weakcoherence}, built upon three principles: (1) keep shared memory globally incoherent to avoid scalability problems and simplify hardware; 
  (2) rely on each node's existing hardware mechanisms to provide local coherence for shared memory, creating ``federations'' of coherent domains that change over time; and
  (3) handle cross-node coordination in software through distributed data structures that navigate the complexities of switching coherence federations.
By shifting complexity to software, we allow specialization of the coordination level required for specific data structures.
At the same time, by leveraging efficiently implementable local coherence, our proposal assists---to the greatest practical extent---multiple cores to continue simple collaborations over shared memory.

Although this approach is a tradeoff between hardware and software implementation complexity, distributed data structures designed for this style of `non-uniform cache coherence' are a tailored fit for efficient exploitation of memory sharing for a wide range of distributed systems.
For example, distributed applications that leverage microservices or pub/sub systems generally use RPCs to share data, which incur serialization and data duplication overheads (even with zero-copy network stacks, as memory is fundamentally duplicated on sender and receiver).
%Pub/sub systems rely on intermediary brokers to relay messages between publishers and subscribers, a process that also entails heavy RPC interaction.
By leveraging shared memory with federated coherence, messages can be stored and distributed with lower latency and higher throughput.
Similarly, immutable shared key-value stores used in distributed compute frameworks (e.g., Apache Ray) could reduce the overhead and inefficiencies of sharing objects by placing them in shared disaggregated memory and provide a path towards reducing object spilling~\cite{ray_spilling}.
In each of these use cases, data structures built atop federated coherence can still exploit local hardware coherence for easier coordination within hosts while still allowing cross-host data coordination.

Overall, by removing the overheads of global coherence and focusing on local coherence domains, our proposal requires simpler hardware, offers better scalability, and is realizable by careful distributed data structure design.
We believe federated coherence for shared disaggregated memory is a practical path toward realizing practical deployments of shared disaggregated memory, and improving modern distributed systems that intensively share data.

%\noteion{The argument of cache coherence is too expensive for multi\-core is expensive -> multi\-node is obvious. But natural question is what are we going to lose if we drop cache coherence in disaggregated memory?}
%\notejae{I gave him some current examples of disaggregated memory use cases and they need minimal coordination across the nodes. He thinks we should put this earlier in the paper to address the question (what will happen if we lose cache coherence). Also as Ion is not as familiar as us in disaggregated memory, he wanted to see the real/practical use cases of disaggregated memory and consequence of no cache coherence }

%find that cache coherence
%  is too costly when
%  disaggregated memory scales to a rack of 20--80 hosts.  
%We argue that the prevailing focus on implementing full,
%    hardware-managed cache coherence across the entirety of a disaggregated memory pool is
%    potentially over-engineered, unnecessarily complex,
%    and could significantly delay the widespread adoption of this transformative technology,
%    ultimately limiting its potential benefits.
%The key insight lies in recognizing the inherent locality often present 
%    in applications and workloads. 
%In many scenarios, cores residing within the same physical node are far more likely to
%collaborate intensively on shared data than cores located on disparate nodes. 
%This observation forms the foundation of our proposed model: \emph{\weakcoherence}.
%Under this model,  each node operates as an independent "coherence domain", where cores within
%    the same node maintain a fully coherent view of the disaggregated memory attached to that node
%    leveraging existing hardware mechanisms. 
%Beyond these boundaries, no coherence guarantees are provided 
%    between nodes accessing shared memory.
%This approach, in essence, creates "federations" of coherent domains,
%    each encompassing a single node.
%Federated Coherence has the potential to be a free lunch from a hardware implementation
%    perspective, as it leverages existing intra-node coherence mechanisms 
%    and avoids the complexity of inter-node coherence across the entire disaggregated pool.
%Having a precisely defined intrinsic coherence model for a disaggregated model will foster
%software developers to write correct software. 
%While requiring some adaptations, the added complexity can be effectively contained within
%    synchronization and shared data structure libraries,
%    minimizing the burden on application developers while enabling significant gains in
%    scalability and performance at the system level.

==> Texts/old/Sec2_Background1.tex <==
\section{Background}
\label{sec:background}

\subsection{Disaggregated Memory}
Disaggregated Memory consists of memory placed outside hosts that they can access through an interconnect.
We consider a disaggregated memory that is directly addressable by processors via load and store instructions,
  rather than mechanisms such as RDMA or page faults.
We are interested in building distributed systems where hosts use disaggregated memory to share
  data.
There is a longstanding debate about whether message passing or shared memory is the best way to build distributed systems. We do not take a position on this debate; instead, we note that disaggregated memory provides an effective way to scale 
   up an application using commodity hardware, by running threads across hosts that share data in disaggregated memory.
Early disaggregated memory deployments have 8--16 sockets~\cite{pond}; the future will see larger
systems with 20--80 servers using CXL v3 switches~\cite{cxl}.

% In this paper, we focus on distributed systems that use shared disaggregated memory\footnote{In this paper,
%   the term (shared) disaggregated memory refers to
%   memory addressable by 
%   load and store instructions, as opposed to mechanisms such as
%   RDMA or page faults (which are less concerned
%   about cache coherence).} for communication. There is a longstanding debate about whether message passing or shared memory is the best way to build scalable systems. We do not take a position on this debate; instead, we note that existing hardware has made it feasible to build shared memory systems using off-the shelf parts. At the same time, the increasing memory demands of modern workloads, and a slowdown in the
%   improvement of local memory capacity has led to increased adoption of disaggregated memory systems. These systems allow multiple servers to combine their compute power to
%   process data placed on large pools of shared memory, and could 
%  provide the computational capacity of an expensive scale-up supercomputer~\cite{nvidia_dgx_gh200} using commodity hardware.
% While early disaggregated memory deployments have 8--16 sockets~\cite{pond}, we envision future rack scale
% system with 20--80 servers using CXL v3 switches~\cite{cxl}.

Disaggregated memory is not a new concept~\cite{LCMRRW2009}
  but recently, several technologies have emerged
  to support it, including CC\-IX~\cite{ccix}, Gen-Z~\cite{genz},
  OpenCAPI~\cite{opencapi}, and more recently CXL~\cite{cxl}.
CXL is now the dominant approach as it has
  become an industry standard with broad
  support from hardware vendors.

\subsection{Issues with Cache Coherence}
\label{subsec:unscalable}

Conventional wisdom says that shared memory should be cache coherent~\cite{MHS2012}, meaning that
  CPU caches must be kept consistent with each other (e.g., the same address cannot be cached at different
  CPUs with different data).
Cache coherence is prevalent (e.g., every x86 server is cache coherent) and easy to understand and program with.
For this reason, CXL is being designed to provide cache coherence of disaggregated memory, by introducing
  back invalidation requests and snoop filters~\cite{backInvalSnoopCaches}.
Roughly speaking, the snoop filter is a mechanism in a CXL memory device that tracks which hosts may be
  caching a location, and when the CXL device sees updates to that location, it sends a back invalidate request
  to those hosts to invalidate their caches.
This is similar to directory-based coherence~\cite{}, but it is coarser grained: the CXL device tracks only
  at the granularity of hosts not individual CPU caches---it is up to each host to find the relevant
  CPU caches when it receives a back-invalidate message.



Achieving full cache coherence in CXL-based disaggregated memory systems necessitates complex hardware mechanisms that introduce significant overheads, potentially hindering scalability and performance.
Indeed, although the CXl3.0 specification describes a cross-node cache coherence protocol as part of cxl.cache, the protocol is incomplete~\cite{cxlformalising} 
and it is unclear whether it can actually scale.
In particular, maintaining a unified view of memory across disaggregated memory nodes generally requires one of two approaches.

The first is snooping, an approach that typically requires broadcasts of coherence messages (e.g., invalidations or updates) to all nodes in the system.
The scalability limitations of this approach are well known, particularly when considering bandwidth overheads.
Snooping is often implemented with the help of snoop filters, which demand substantial on-chip SRAM capacity and sophisticated lookup and update logic.
The complexity of managing and querying these filters also grows exponentially with the number of coherent agents~\cite{AMDCXL}.

The second is distributed directory which is more common in larger systems.
However, although directories mitigate snooping traffic, they introduce their own overheads, 
including inter-node directory lookups across the CXL fabric, the implementation of intricate directory coherence protocols, and the incorporation of mechanisms for fault tolerance~\cite{sdm}. 
These inherent hardware complexities are compounded by the non-negligible latency associated with accessing remote memory over the CXL interconnect and potential bandwidth saturation on the fabric.

%In particular, scaling cache coherence to large core counts and across disaggregated memory nodes requires broadcasts or complex directory management to maintain a unified view of memory.

%As the number of coherent agents grows, the overhead of snooping or traversing extensive directory structures to track data ownership and ensure consistency becomes prohibitively expensive in terms of latency and bandwidth.

%\notejae{rephrase that it isn't incomplete but needs more formal proof yet.}

%Maintaining consistency across a potentially large number of coherent agents requires intricate solutions such as large-scale on-chip snoop filters or distributed directory protocols.

These factors create bottlenecks, particularly for fine-grained sharing and frequent data exchanges,
leading to a fundamental trade-off between coherence and performance in disaggregated memory architectures.
Consequently, current CXL memory solutions and prototypes typically forgo full cache coherence.



%\notevincent{compress:}
\notevincent{say that current hardware just doesn't support it.}

Recent proposals have even called for segregated memory layouts.
\notevincent{This whole section sets up Pasha to look too much like our approach.  The emphasis should be on the fact that they divide memory into two extremes (and that will be insufficient)}
For example, Pasha~\cite{pasha} adopts a pragmatic approach to memory consistency in CXL pods.
Instead of striving for a globally coherent shared memory space across all CXL-attached devices, Pasha divides memory in two: local memory (within the server node) and remote memory (attached via CXL). 
Local memory maintains strong cache coherence, while memory accessed through CXL devices typically has weaker consistency guarantees.

The onus of maintaining data integrity and consistency for CXL memory largely falls on the database system itself.
Pasha leverages application-level knowledge and control, potentially employing strategies like epoch-based consistency where the database tracks changes within defined epochs and ensures consistency at epoch boundaries. 
This allows for efficient access to CXL memory for bulk data operations or as a larger, less frequently accessed storage tier.
The database can explicitly manage data movement and synchronization between local and CXL memory when necessary, avoiding the continuous overhead of hardware-enforced cache coherence across the entire disaggregated pool. 

\notejae{daniel berger's talk. Please pass me daniel's slides if he replies}

The challenges of achieving scalable cache coherence are not unique to CXL-based systems. 
Insights from many-core processors highlight evolving strategies for managing coherence in complex environments, offering valuable precedents for disaggregated memory architectures.
In many-core architectures, processors are often organized into clusters or tiles of cores to improve performance and scalability. 
This structure naturally lends itself to a hierarchical approach to coherence.
Within a cluster, a traditional full coherence protocol (like MESI or MOESI) is typically employed to maintain consistency between the caches of cores that share a lower-level cache (e.g., L2). 
Beyond the cluster, coherence protocols are layered to reflect varying access latencies: 
cores sharing an L3 cache within a NUMA node maintain stricter coherence,
while coherence across physical sockets or the entire system is progressively relaxed.

The hierarchical approach to coherence, particularly in NUMA systems,
    demonstrates a clear move towards more nuanced and localized coherence strategies. 
It reflects the growing need to manage complexity and communication costs in large multi-core architectures—challenges 
that are significantly amplified in the context of disaggregated memory systems.



\subsection{Beyond Black and White}

The nascent landscape of disaggregated memory demands a more nuanced approach to coherence than the current ``all or nothing'' paradigm. 
The simplistic dichotomy of full coherence versus no coherence at all fails to capture the rich spectrum of possibilities that lie between these extremes.
We must move beyond binary thinking and embrace coherence models that strike a pragmatic balance. Locality,
rather than global uniformity, is the key to unlocking the full potential of disaggregated memory.

\heading{The Limits of "All or Nothing".} At one extreme of the spectrum lies the fully non-coherent model. 
In this scenario, no hardware support for coherence is provided across any of the cores accessing the disaggregated memory. 
While this approach minimizes hardware complexity, it shifts an enormous burden of managing consistency to software developers who have to use mechanisms like message passing or remote memory operations (e.g., RDMA). 
This manual management can be error-prone, difficult to debug,
and unsuitable for general-purpose applications. 
While certain High-Performance Computing (HPC) workloads with well-defined communication patterns may tolerate such a model,
it is an impractical choice for broader adoption.

At the other end of the spectrum is the fully coherent model, which guarantees a globally consistent view of the disaggregated memory across all cores in the system. 
This is the most straightforward model for software developers, as it mirrors the familiar shared-memory paradigm of traditional SMP systems.
However, as discussed in ~\cref{subsec:unscalable}, achieving full coherence across a large-scale disaggregated system presents significant hardware design challenges and may incur substantial performance overhead due to the communication required to maintain consistency across a large number of nodes.
Several disaggregated memory usecases (described in ~\cref{sec:casestudy}) do not require coherent view most of the time.
However, full cache coherence guarantees incur coherence traffic across all nodes even if there's no sharing at all.
It can be exacerbated if nodes working separately on different regions of the disaggregated memory have false sharing where
they do not shared memory regions but their working space overlap within a cacheline.
As systems grow, the overhead of maintaining global coherence becomes untenable,
particularly for workloads with high data-sharing frequency or fine-grained memory access patterns.

\heading{The Case for Federated Coherence.}
\notejae{key idea is rely on h/w for frequent coordination which happens within a node and manual coordination for rare sync across nodes to reduce h/w complexity and performance for maintaining full coherence.}
The inadequacies of these extremes make it clear that the future of disaggregated 
memory requires a middle ground—a model that balances performance, scalability,
and complexity while respecting the inherent locality of data access.
This is where Federated Coherence excels.
Federated Coherence breaks free from the all-or-nothing paradigm by introducing a hierarchical and localized approach to coherence.

\notevincent{heirarchical processing (dbs, spark, ray) -> pointer transfers}

In Federated Coherence, each node becomes a "federation" of coherence. 
Within a single node, cores maintain a fully coherent view of the disaggregated memory attached to that node,
leveraging well-established intra-node coherence mechanisms. 
However, coherence guarantees do not extend across nodes accessing the same disaggregated memory.
This design choice avoids the complexities and overheads of inter-node coherence protocols, while still enabling efficient and fully coherent data sharing within each node.

\heading{Why does it work?}
Federated Coherence is grounded in the observation that data locality is a dominant characteristic of many workloads.
By prioritizing local coherence within a node,
Federated Coherence enables efficient data sharing and communication where it is most needed,
while avoiding the prohibitive costs of global coherence.
This model offers several key advantages:
First, Performance through Locality. 
Applications with data-sharing patterns that are primarily confined to a single node benefit from the high performance of intra-node coherence mechanisms. 
Each node can maintain local caches of frequently accessed data, minimizing costly remote memory operations.
Second, Simplified Software Development. 
Within a node, developers can rely on fully coherent memory,
simplifying parallel programming and enabling the use of familiar shared-memory paradigms. 
Thread pools within a node can safely and efficiently share data without requiring explicit synchronization mechanisms.
Third, Reduced Hardware Complexity.
By limiting coherence to the node level,
Federated Coherence avoids the need for complex inter-node coherence protocols,
snooping mechanisms, or directory lookups across the CXL fabric.
This simplifies hardware design and reduces scalability bottlenecks.
Fourth, Adaptable Software Abstractions.
While Federated Coherence requires software to be aware of coherence boundaries,
this complexity can be encapsulated within libraries or middleware.
Developers can work with high-level abstractions that hide the underlying coherence model,
minimizing disruption to application code.
Fifth, Scalability.
By decoupling coherence between nodes, 
Federated Coherence supports larger, more scalable disaggregated systems.
The localized coherence model reduces inter-node communication overhead,
making it well-suited for systems with high node counts or diverse workloads.

==> Texts/old/Sec3_Definition1.tex <==
\section{\WeakCoherence}
\label{sec:newcoherence}


The nascent landscape of disaggregated memory demands a more nuanced approach to coherence than the current black-or-white paradigm. 
The simplistic dichotomy of full coherence versus no coherence at all fails to capture the rich spectrum of possibilities that lie between these extremes.
We must move beyond binary thinking and embrace coherence models that strike a pragmatic balance. Locality,
rather than global uniformity, is the key to unlocking the full potential of disaggregated memory.


\heading{The Case for Federated Coherence.}
\notejae{key idea is rely on h/w for frequent coordination which happens within a node and manual coordination for rare sync across nodes to reduce h/w complexity and performance for maintaining full coherence.}
The inadequacies of these extremes make it clear that the future of disaggregated 
memory requires a middle ground—a model that balances performance, scalability,
and complexity while respecting the inherent locality of data access.
This is where Federated Coherence excels.
Federated Coherence breaks free from the all-or-nothing paradigm by introducing a hierarchical and localized approach to coherence.

\notevincent{heirarchical processing (dbs, spark, ray) -> pointer transfers}

In Federated Coherence, each node becomes a "federation" of coherence. 
Within a single node, cores maintain a fully coherent view of the disaggregated memory attached to that node,
leveraging well-established intra-node coherence mechanisms. 
However, coherence guarantees do not extend across nodes accessing the same disaggregated memory.
This design choice avoids the complexities and overheads of inter-node coherence protocols, while still enabling efficient and fully coherent data sharing within each node.

\heading{Why does it work?}
Federated Coherence is grounded in the observation that data locality is a dominant characteristic of many workloads.
By prioritizing local coherence within a node,
Federated Coherence enables efficient data sharing and communication where it is most needed,
while avoiding the prohibitive costs of global coherence.
This model offers several key advantages:
First, Performance through Locality. 
Applications with data-sharing patterns that are primarily confined to a single node benefit from the high performance of intra-node coherence mechanisms. 
Each node can maintain local caches of frequently accessed data, minimizing costly remote memory operations.
Second, Simplified Software Development. 
Within a node, developers can rely on fully coherent memory,
simplifying parallel programming and enabling the use of familiar shared-memory paradigms. 
Thread pools within a node can safely and efficiently share data without requiring explicit synchronization mechanisms.
Third, Reduced Hardware Complexity.
By limiting coherence to the node level,
Federated Coherence avoids the need for complex inter-node coherence protocols,
snooping mechanisms, or directory lookups across the CXL fabric.
This simplifies hardware design and reduces scalability bottlenecks.
Fourth, Adaptable Software Abstractions.
While Federated Coherence requires software to be aware of coherence boundaries,
this complexity can be encapsulated within libraries or middleware.
Developers can work with high-level abstractions that hide the underlying coherence model,
minimizing disruption to application code.
Fifth, Scalability.
By decoupling coherence between nodes, 
Federated Coherence supports larger, more scalable disaggregated systems.
The localized coherence model reduces inter-node communication overhead,
making it well-suited for systems with high node counts or diverse workloads.

\heading{Definition}
We define \weakcoherence following two common practices in coherence definitions~\cite{SWD2011}.
First, coherence is defined separately from the memory model,
  by considering the order of operations issued by processors to the cache
  controller rather than the program order.
  %(which may allow instruction re-ordering and other
  %quirks)---thus, the coherence definitions are with respect to the
  %order of operations issued by the processors
  %to the cache or memory controller, rather than
  %the program order.
% Second, the definitions cover only load and store operations
%   not read-modify-write operations (compare-and-swap, fetch-and-add, etc).
Second, coherence is defined for a single fixed memory location rather than the entirety of memory.
%
We start with the standard 
  cache coherence definition~\cite{SWD2011},
  where memory operations are 
  $\t{write}_p(v)$ and $\t{read}_p(v)$, 
  representing a store and load of $v$ 
  by processor $p$ at a fixed memory location.

\begin{definition}
\label{def:coherence}
  A memory system satisfies \emph{cache coherence} if, for every execution and each memory location $\ell$, there is a total order $\mathcal{O}$ of operations on $\ell$ in the execution, such that:

  \begin{enumerate}
  \item $\mathcal{O}$ is consistent with the order of operations on $\ell$ issued by each processor $p$.%\notepanda{Order of operations makes this sound like we are assuming SeqCst? Maybe issued is the problem?}

  \item In $\mathcal{O}$, a read $r$ returns the value of the last write that precedes $r$.
  \end{enumerate}
\end{definition}

\noindent For convenience, we assume that the execution
starts with $\t{write}_{p_0}(v_0)$, representing
the initialization value $v_0$ of $\ell$ by a
hypothetical processor $p_0$.
%
Thus, Definition~\ref{def:coherence} states that operations on a memory location can be serialized,
such that a read always
returns the value of the latest write.
%(where the
%serialization may differ from location to location).

For weaker forms of coherence, we extend processor operations
  to include $\t{flush}_p$, 
  representing a flush of the cache of processor $p$ to memory.
%
  % \noteamaro{Can we unify the definition of flush to always flush from a shared cache? I believe this modified condition doesn't require us to make the flush here only apply to processor p's cache. This would allow us to have a single definition of flush}
  % \notemarcos{if we use a single shared cache in this definition, we get full coherence because caches cannot diverge}
%  
We now define a system with
  a weak form of coherence where processors
  can explicitly flush their caches.
This definition is obtained by modifying condition (2) in Definition~\ref{def:coherence} as follows:

{\it
  \begin{enumerate}
  \item[(2)] In $\mathcal{O}$, a read $r$ returns a
  value picked as follows:

  \begin{enumerate}
      \item If the last operation by $p$ preceding $r$ is $\t{write}_p(v)$ or $\t{read}_p(v)$, pick value $v$.

      \item If the last operation by $p$ preceding $r$ is
      $\t{flush}_p$,
%
\eat{
      $r$ returns the value $v$ from the last $\t{write}_q(v)$
      preceding the most recent $\t{flush}_q$ by any processor $q$.\noteamaro{check--original eaten below}
      \notemarcos{the notion of ``most recent'' isn't
                 clear.}
}
      find the process $q$ with the
      last $\t{flush}_q$ preceding $r$
      %(this could be $q=p$)
      and pick the value $v$ from the
      last $\t{write}_q(v)$ preceding the $\t{flush}_q$.

  \end{enumerate}

  \end{enumerate}
}

Intuitively, this condition says that a read should
 return either the value in the local cache or the
last value that was flushed to memory, depending on whether the reading processor recently flushed its cache.
For convenience, we assume the execution
starts with $\t{write}_{p_0}(v_0)$ followed by $\t{flush}_p$ for every processor $p$.
%\notevincent{the initialization probably needs updating here (fake flush)?}

\eat{
  We next give a definition of \weakcoherence
  where
  all flushes are explicitly issued by the
  program (no cache eviction by the system).
  We obtain this definition by replacing condition (2) of Definition~\ref{def:coherence} with the following:

  {\it
  \begin{enumerate}
  \item[(2)] In $\mathcal{O}$, a read $r$ returns one of the following:

  \begin{enumerate}
      \item If the last operation by some process $p'\in\t{node}(p)$ preceding $r$ is $\t{write}_{p'}(v)$ or $\t{read}_{p'}(v)$, pick the value $v$.

      \item If the last operation by some process $p' \in \t{node}(p)$ preceding $r$ is
      $\t{flush}_{p'}$, find the process $q$ with the
      last $\t{flush}_q$ preceding $r$ and pick the value $v$ from the
      last $\t{write}_{q'}(v)$ preceding the $\t{flush}_q$ with $q'\in\t{node}(q)$.
  \end{enumerate}

  \end{enumerate}
}
}

We now 
  define \weakcoherence
  by modifying the previous definition in two ways.
First, we extend the cache to be shared by all the processors in a node,
  where the intended behavior of a $\t{flush}_p$ operation is to flush this shared cache.
%\noteamaro{should we explicitly say this was not true before?}
%MKA: done, we now say earlier that flush_p represents a flush
%of the cache of processor p.
Second, we allow the total order $\mathcal{O}$
  to include additional flush operations not
  present in the execution,
  representing cache evictions by the hardware.
  %\noteamaro{what system?}.

\begin{definition}
\label{def:weakcoherence}
  A memory system satisfies \emph{\weakcoherence} if, for every execution
  and each memory location $\ell$, there is   
  a total order $\mathcal{O}$ that includes all
  operations on $\ell$ in the execution and
  possibly additional $\t{flush}$ operations, such that:

  \begin{enumerate}
  \item $\mathcal{O}$ is consistent with the
      order of operations on $\ell$ issued by each processor $p$.

  \item In $\mathcal{O}$, a read $r$ returns a value picked as follows:

  \begin{enumerate}
      \item If the last operation by any processor $p'\in\t{node}(p)$ preceding $r$ is $\t{write}_{p'}(v)$ or $\t{read}_{p'}(v)$, pick $v$.

      \item If the last operation by any processor $p' \in \t{node}(p)$ preceding $r$ is
      $\t{flush}_{p'}$,
\eat{
      then $r$ returns the value $v$ from the last $\t{write}_{q'}(v)$ preceding the most recent $\t{flush}_q'$ by any processor $q'$, where $q' \in \t{node}(p)$.\noteamaro{check--original eaten}
}
      find the process $q$ with the
      last $\t{flush}_q$ preceding $r$ and pick the value $v$ from the
      last $\t{write}_{q'}(v)$ preceding the $\t{flush}_q$ with $q'\in\t{node}(q)$.
      \eat{\notepanda{This one is a bit strange. What happens when $p, q\in \t{node}(p)$?}
      \notemarcos{$p$ is always in $\t{node}(p)$, so nothing different
      happens. If $q \in \t{node}(p)$, this corresponds to
      the node flushing its cache then reading again from memory.}
      \notepanda{Also what happens if $\t{node}(p)$ does not have the location cached,
      and also does not issue a flush?}
      \notemarcos{Impossible. If the location is not cached, it's
      because a flush happened by the program or due to
      an eviction (that's why $\mathcal{O}$ may include additional
      flush operations)}
      \notepanda{Also, if $\t{node}(p) = \t{node}(q)$, and there is a $\t{write}$ from $\t{node}(q)$ between $\t{flush}_q$ and $r$, do we loose the write?}
      \notemarcos{Impossible. That falls in case (a) above not (b).}}
  \end{enumerate}

  \end{enumerate}
\end{definition}

\noindent Here $\t{node}(p)$ denotes the set with the processors
in the same node as $p$, and
%\noteamaro{Can we add an intuitive summary of def 2?}
$\t{flush}_p$ is an operation by $p$ to
  flush the cache shared by processes
  in $\t{node}(p)$.
Intuitively, Definition~\ref{def:weakcoherence} says that in the serialized order, reads should return either the value in the cache shared by the node, or the last value flushed to memory from one of the shared caches, depending
on whether the reader's shared cache has been flushed.
%by a process in the reader's node.

% The above definition covers only loads and stores but it is
%   easy to extend it to read-modify-write
% operations (\eg compare-and-swap, fetch-and-add).
% \notemarcos{does it make sense for the processor to issue atomic
% operations to the cache or memory controller?}


\heading{Anomalies.}
\label{sec:anomalies}
%
With \weakcoherence, two types of anomalies are possible:
  cross-node stale reads and cross-node broken atomicity.
Cross-node stale reads happen when a read 
  runs at a node different from the one that
  issued the last preceding
  write, causing the read to miss the write and
  return a stale value.
Cross-node broken atomicity happens when
  atomic operations run at two different nodes
  causing them to break their atomic behavior (e.g.,
  two compare-and-swap atomics may succeed when only one was supposed to, or two fetch-and-increment atomics may increment a counter by only one).
These anomalies break existing concurrent data
  structures (e.g., lock-free queues), synchronization primitives
  (e.g., locks, semaphores), and consistency guarantees
  expected by most developers 
  (e.g., release consistency\footnote{Release consistency ensures that modifications done while a lock is held
  become visible to subsequent lock holders.}).

However, with \weakcoherence, such anomalies happen
  only across nodes.
If a read runs on the same
  node as the last preceding write, the read
  returns the correct value.
If two atomic operations run on the
  same node, they preserve their atomic guarantees.
These guarantees are the basis for writing
 application libraries under \weakcoherence (\S\ref{sec:proposal}).

\eat{
\subsection{Implementation}

\notevincent{Since we're over on space, this subsection is a candidate for deletion.}\notepanda{I agree, deleting this if necessary seems fine.}
While a complete design for hardware that provides disaggregated memory with \weakcoherence is well beyond the scope of this paper, here we briefly sketch a possible approach.
The basic idea is that each node runs its internal hardware-based
  coherence protocol as provided in modern processors.
We connect all nodes to the disaggregated memory without additional coherence mechanisms so that when a node flushes its cache to memory, it immediately overwrites the previous contents without coordinating with other
  caches.
Note this implementation is efficient because the coherence traffic is constrained within each node.
% \notevincent{This section is a bit sparse.  Is there anything else we can add? If no time, it's fine to keep as is.}
}

\eat{
We focus on the CXL v3 hardware
  as the leading contender to realize shared
  disaggregated memory.
  \notepanda{Is there a particular thing we do
  in the proposal below that relies on anything from CXLv3?
  Especially given we disable the coherence engine?}
As we explained before, CXL v3 provides (full)
  cache coherence
  through back-invalidate messages from the disaggregated
  memory controller (home agent).
Basically, we obtain a system with \weakcoherence by
  omitting such messages and the snoop filter mechanism that
  supports them.
\notemarcos{Emmanuel: isn't there a way to disable
cache coherence in CXL (e.g., by definition regions
that are not coherent)? How did that work?}\noteamaro{The spec says regions can have software-defined coherence. I think the way it worked in Niagara is, they just exposed the regions to multiple hosts and that's it}
}

\endinput

\begin{outline}
\0 background on cache coherence
    \1 cache coherence enables consistent sharing of data in multicore processors
    \1 from first principles: here's where the scaling problem comes from
    \1 cache coherence vs memory model (TSO)
        \2 cache coherence only talks about caches but not about store buffers
    \1 memory fences

    
\0 CXL cache coherence: Back invalidate snoop
    \1 this will still be bad
    \1 CXL spec allows incoherence: software-managed coherence

\0 what does incoherence means
    \1 lock instructions and atomics don't work
    \1 what is TSO under incoherence
    

\0 (not sure if this should go here) CXL vs NVLink
\end{outline}

==> Texts/old/Sec4_CaseStudy1.tex <==
\section{Using Federated Coherence}
\label{sec:casestudy}

Federated Coherence introduces a novel coherence model tailored for multi-node disaggregated memory systems.
By maintaining full coherence within individual(usual case) nodes but avoiding inter-node(rare case) coherence complexities,
    this model strikes a balance between performance, simplicity, and programmability.
To demonstrate the versatility and effectiveness of Federated Coherence,
    we first outline general techniques and synchronization mechanisms that work seamlessly within this paradigm.
We then explore specific use cases where Federated Coherence provides significant advantages, showcasing its potential to address diverse workloads efficiently.

\heading{General Techniques for Synchronization Without Cache Coherence.}
While Federated Coherence deliberately avoids hardware-level inter-node coherence,
    software-level mechanisms can readily bridge this gap,
    enabling efficient communication and data sharing between nodes.
These techniques often involve explicit synchronization and awareness of the coherence boundaries.

Several \textit{Distributed Locks} techniques were studied that could work in between non-coherent domains like Lamport's Bakery Algorithm~\cite{bakery}, modified Peterson's lock~\cite{petersons}, token based locks~\cite{wagner2000token}, etc.
\textit{Conflict-Free Replicated Data Types(CRDT)} data structures allow concurrent updates from multiple nodes without requiring strict synchronization. 
Updates are merged using mathematical properties, ensuring eventual consistency.

There exists \textit{Task-Based Paradigms and Immutability} where workloads have inherent immutability (e.g., immutable object stores).
Cross-node coherence is unnecessary once data is written.
References to immutable data can be safely passed across nodes without additional synchronization.

With \textit{Versioning and Epoch-Based Consistency},
    nodes explicitly mark shared data as ready or updated using version numbers or epochs.
This ensures readers in other nodes observe a consistent view of the data.
\textit{Ownership} of data blocks can be explicitly assigned to nodes, 
    allowing synchronization at logical boundaries (e.g., partitions or segments in memory).
Consider a shared memory region $m$ accessible by $i$ servers, 
    each possessing a local memory view $v_i$.
At any given time, only one memory view, denoted as $v_owner$, 
    maintains coherence with the global shared memory $m$.
The remaining views are considered temporarily incoherent with $m$, 
    and importantly, no two local views $(v_i, v_oj)$ are mutually coherent.
When a node possesses ownership, all cores within that node can leverage standard intra-node cache
    coherence mechanisms for efficient and consistent access to $m$.
Crucially, atomic operations performed within the owning node operate correctly on $m$.
Mechanisms for managing ownership transitions,
    such as explicit ownership transfer protocols, versioning schemes,
    or epoch-based synchronization, are integral to this model. 
These mechanisms ensure that coherence is maintained when ownership is switched.

%\notejae{You select a region of shared memory m, each with one memory view v\_i for i servers that can access m. A memory view can be coherent or incoherent with m, but this can change over time. Only one v\_i will be coherent with m out of all the v\_i at one time, the rest will be incoherent. In addition, no v\_i and v\_j are coherent with each other.If v\_i is currently coherent with m, all cores in the server i can use local coherence to access m, in particular, atomics from v\_i work correctly with m. Mechanisms like ownership, versioning, and epochs can fit well with federated coherence and can be used to switch the memory view currently coherent with m. For example, with ownership, the currently coherent v\_i is the owner, and we can switch ownership to v\_j. If very frequent ownership change happens, v\_i and v\_j can use a memory location to indicate ownership change, and the one who isn't an owner polls the memory location (with cache flush). If infrequent ownership change happens, v\_i can send a message to v\_j (via network or CXL.io)}

%The frequency of ownership changes dictates appropriate implementation strategies. 
%Shared memory location can act as an ownership flag for frequent ownership transfers. 
%The non-owning node can efficiently monitor this flag (potentially employing cache line invalidation or flushing to ensure up-to-date reads) to detect ownership changes.
%In cases of infrequent ownership transfer, a message-passing approach, leveraging the underlying network fabric or CXL.io, can be employed to signal ownership transitions, minimizing unnecessary polling overhead. This adaptive approach to ownership management allows Federated Coherence to optimize performance based on workload characteristics.

These techniques provide a foundation for effective synchronization in Federated Coherence-enabled systems, enabling various applications to leverage its benefits. 
By leveraging Federated Coherence alongside these synchronization mechanisms,
disaggregated systems can achieve scalable performance while maintaining a manageable level of complexity.
These case studies demonstrate the versatility of Federated Coherence,
    making it a practical and effective model for a wide range of applications.

\heading{Compelling Use Cases for Federated Coherence.}
These representative usecases highlight how Federated Coherence strikes a compelling balance between performance,
complexity, and programmability, making it a viable solution for diverse workloads.
\paragraph{Microservice}
,often leverage Remote Procedure Calls (RPCs) to communicate.
Disaggregated memory can be used to efficiently pass the payload of these RPC calls
    (as preliminarily demonstrated by ~\cite{dmrpc,hydrarpc}),
    allowing the receiving service to directly operate on the data in place.
Since the data payload in disaggregated memory is typically accessed exclusively by the receiver,
    Federated Coherence provides sufficient coherence within the receiving node for processing the request.
This avoids the need for explicit data copies or complex coherence protocols, reducing latency and improving throughput. 

Cross-node synchronization can be achieved using versioning or epoch-based consistency.
The sender marks the payload as ready, allowing the receiver to see a consistent view of the data.
This avoids the need for complex inter-node coherence protocols, reducing latency and improving throughput.

\paragraph{Shared Log}
, commonly used in publish/subscribe systems or distributed databases, 
    align naturally with the boundaries of Federated Coherence.
In these systems, individual nodes typically write to their designated log partitions, while other nodes read the logs.

For example, in a publish/subscribe system, publishers append messages to their local log partitions,
    and subscribers on other nodes read the messages.
Federated Coherence ensures full coherence for publishers within their local nodes,
    enabling efficient log updates.
Subscribers, on the other hand, read the logs without requiring strict inter-node coherence.

To ensure data visibility between nodes, explicit synchronization mechanisms,
    such as an owner bit or coherence-free mutexes, can be employed at log boundaries. 
These techniques eliminate the overhead of maintaining full coherence for read-only operations, 
    making shared log systems an ideal use case for Federated Coherence.

\paragraph{Immutable Object Stores}
are often used in distributed system frameworks like Ray.
Once an object is written by a task or actor (which may be multi-threaded), it becomes immutable.
Frameworks then pass references to these objects, and tasks or actors retrieve them as needed.
The immutability of the objects eliminates the need for strict cross-node coherence once the object is written, making Federated Coherence a suitable model.

\paragraph{Memory pooling}
refers to where disaggregated memory is allocated as exclusive regions to individual Virtual Machines (VMs).
Whether treated as an extension of local memory (e.g., through memory tiering) or as a separate pool,
    Federated Coherence ensures full coherence for cores within the VM's allocated region.

For example, a VM accessing its assigned region of disaggregated memory benefits from intra-node coherence, 
    enabling efficient data access and manipulation. 
Since the allocated region is primarily accessed by the owning VM, cross-node coherence is unnecessary.
This simplifies the memory management model while maintaining high performance.

==> Texts/old/Sec5_CallToAction1.tex <==
\section{The Path Forward: Call to Action}
\label{sec:calltoactions}
\notepanda{highlight major takeaway: we need to have discussion now, in future it will be a bigger problem and untenable}

\topheading{For hardware vendors.}
Leverage Existing Intra-Node Coherence, a ``Near Free Lunch.''
Federated Coherence leverages existing intra-node coherence mechanisms already present in modern processors and interconnects.
This means that significant portions of the necessary hardware infrastructure are already in place.
The "near free lunch" aspect comes from repurposing these existing mechanisms for a new purpose: establishing clear coherence boundaries at the node level.
This avoids the need for entirely new, 
    complex inter-node coherence protocols across the entire disaggregated memory pool.
It's not that the hardware fully implements Federated Coherence today,
    but rather that it provides the essential building blocks, making it a relatively low-cost and quick-to-implement solution. 
The key is to define and expose these node-level coherence domains to software.
Prioritize Time-to-Market.
Implementing full hardware coherence across a disaggregated memory pool is a significantly more complex undertaking than leveraging existing intra-node coherence.
This complexity translates to longer development cycles, higher costs, and delayed product releases.
By focusing on Federated Coherence, hardware vendors can bring disaggregated memory solutions to market much faster,
enabling early adoption and fostering innovation. 
This quicker time-to-market allows software developers to begin experimenting and developing new applications for disaggregated memory sooner, which, in turn, drives further hardware innovation.

\heading{For software researchers.}
Develop Techniques to Leverage Federated Coherence.
This includes developing new synchronization primitives, data placement strategies, and fault tolerance mechanisms tailored to the node-level coherence boundaries of Federated Coherence. For example, explore techniques like region-based locks, distributed consensus algorithms optimized for Federated Coherence, and data replication strategies that minimize inter-node communication. The use of owner bits managed by coherence-free mutexes, as mentioned previously, is one such example.
Explore Programming Models: Investigate programming models that explicitly expose coherence domains to developers, allowing them to optimize data placement and synchronization. Languages like Rust, with its ownership and borrowing system, provide inspiration for how such models might be designed.
Develop Benchmarks: Create benchmarks that accurately reflect the performance characteristics of different coherence models on disaggregated memory. These benchmarks should consider various workloads, communication patterns, and data access patterns.
Develop Libraries: Create new synchronization and data structure libraries specifically designed for Federated Coherence. These libraries should encapsulate the complexity of inter-node synchronization and data consistency management, providing higher-level abstractions for application developers.

\heading{For the Community.}
Call for Open Discussion and Collaboration: Foster a broader community discussion about the optimal coherence levels for disaggregated memory. Encourage collaborative research efforts between hardware vendors, software developers, and academic researchers. This includes establishing open standards and APIs for interacting with disaggregated memory under different coherence models.


==> hotnets24/S0abstract.tex <==
%\begin{abstract}
\section*{Abstract}

Byte-addressable disaggregated memory will soon be 
  in data centers, aiming to increase memory
  size and bandwidth, improve memory utilization,
  and permit efficient sharing of data between compute nodes.
Current proposals for disaggregated memory 
  plan to provide hardware-based cache coherence similarly to local memory.
However, we find that the cost of coherence becomes
  untenable as disaggregated memory scales to
  many nodes.
We thus introduce a new model of coherence called
  \emph{\weakcoherence}, which leverages the existing hardware coherence
  mechanisms within each node, without incurring the coherence costs across nodes.
We explain how to use \weakcoherence to build
  strongly consistent application libraries that
  developers can use without concern for the weaker
  notion of coherence.

%\end{abstract}

\endinput

Other Potential titles. Place your title here

\paragraph{$\bullet$ Playing the "Devil's Advocate":}
\begin{enumerate}
    \item Rethinking the Coherency: Are we on the right path?
    \item The Incoherent Truth About Memory Disaggregation: Challenging the Status Quo 
    \item Coherency: A Necessary Evil or an Outdated Paradigm?
\end{enumerate}

\paragraph{$\bullet$ Emphasizing a Paradigm Shift:}
\begin{enumerate}
    \item Beyond Coherency: Unlocking New Performance Frontiers in Disaggregated Memory
    \item From Coherency to Coordination: A New Foundation for Disaggregated Memory Systems
    \item Want to Scale Disaggregated Shared Memory? Drop Coherence!!
\end{enumerate}

\textit{$\bullet$ Overcoming the Coherence Barrier in Disaggregated Memory}




==> hotnets24/S1intro.tex <==
\section{Introduction}
\label{sec:intro}

Memory disaggregation is a recent trend in data center design,
  where memory is decoupled from server enclosures and placed
  on a fabric so that it can be accessed by multiple servers.
This architectural shift 
  enhances memory capacity and bandwidth,
  improves memory utilization, 
  and permits efficient data sharing between nodes~\cite{das2023introduction,legoos,aguilera2023memory}---capabilities
  that are crucial for modern workloads that must handle
  and share increasing amounts of in-memory data~\cite{stephanie_ownership, exoshuffle, ramcloud, spark, rdds, graphx}.
%
% Recent memory disaggregation proposals (e.g., as in 
%    Compute eXpress Link (CXL)~\cite{cxl})
%   offer a CPU load-store interface with
%   \emph{cache coherence}, ensuring CPU caches 
%   coordinate to present a coherent view of
%   memory equivalent to local memory, despite disaggregated memory
%   being shared across hosts.
% Cache coherence combined with the use of proper
%   synchronization primitives (atomics, fences, etc.)
%   enables consistent data sharing across threads:
%   if one thread writes to a location, another thread
%   can subsequently observe the written data.
% \notejae{
% What about this version to emphasize that memory disaggregation simply extended existing cache coherent memory semantics?
% Recent memory disaggregation proposals (e.g., as in 
%    Compute eXpress Link (CXL)~\cite{cxl}) extend the traditional shared memory model. 
%    In this model, \textit{cache coherence protocols} ensure that each core maintains a consistent view of the shared memory region, equivalent to local memory despite the memory is shared across hosts.
%    These protocols are used with a combination of synchronization primitives(atomics, fences, etc) to guarantee correctness and prevent data races.
%    By abstracting away the complexities of distributed memory management, cache coherence significantly simplifies programming while facilitating efficient performance across diverse CPU architectures.}
%\notevincent{is it correct to say that it emulates traditional CPU semantics a bit better, enabling access through LD/ST instructions for legacy applications? If so, I think what we're arguing for is to handle correctness at a higher abstraction layer}
%\notemarcos{Yup. I edited the text above to say "provide the same coherent view of memory as local memory does''}
%
%We are particularly interested in using memory disaggregation for sharing data across hosts~\cite{}. VL: repetetive with previous sentence
%\notemarcos{Changed next based on Jae's suggestions, and merged with para 1. Pls chk}
Recent memory disaggregation proposals, such as 
   Compute eXpress Link (CXL)~\cite{cxl}), retain a traditional shared memory model
   with \textit{cache coherence}, whereby
   CPU cores have the same consistent logical
   view of
   disaggregated memory as local memory,
   despite memory being cached and
   shared across nodes.
%Cache coherence combined with the use of
%  synchronization primitives (atomics, fences, etc)
%  guarantee correctness and prevent data races.
Cache coherence hides the
  complexity of distributed cache management and provides a simple programming
  model independent of the
  system architecture.
   

Despite its utility, cache coherence comes at a high price:
  it requires an expensive coherence
  protocol interposed on memory accesses
  %\notepanda{Is `every memory access' a bit overstated here (I guess the question is what we consider the protocol)? I know the truth is more subtle, but I wonder if we want to say something a bit softer?}
  to ensure that caches 
  %and disaggregated memory 
  do not lose updates or serve
  stale data (\S\ref{sec:costcoherence}).
While the costs of cache coherence have been extensively debated in the context of multicore processors~\cite{MHS2012,scaleNUMA}, we argue that hardware-based cache coherence is significantly more expensive for disaggregated memory 
compared to the local memory of a server,
  for two main reasons.
First,
  disaggregated memory systems have a larger
  number of CPUs sharing memory, which is problematic
  as the overhead of coherence increases with the
  number of participating CPUs (\S\ref{sec:background}).
Second, the coherence protocol experiences a larger
  communication latency because components are in different
  nodes.
For example, with CXL disaggregated memory, modifying memory cached in another
  node takes at least two remote round trips:
  one to contact the \emph{home agent} of the cache 
  line in disaggregated memory (essentially a directory),
  %\notepanda{Not opposed, but just flagging, do we want to say most high-core count processors use directory based mechanisms, as a footnote?},
  %MKA: Not clear how that helps the line of argument
  %AP: It was not so much for line of argument, which I agree it doesn't help, but rather to ward off anyone who is thinking of snooping.
  and another for the home agent to 
  ask the other node 
  to invalidate the cache line.
Additional communication is required if the remote cache
  line is dirty.
  


%Even within a host, running a coherence protocol on local interconnects is costly~\cite{onur_ref}~(\S\ref{sec:background}).
% Disaggregated memory makes the situation worse
%   because (1) the coherence protocol is subject to
%   higher
%   latency to communicate over a remote
%   interconnect and (2) the number of CPU caches
%   and hence the coherence traffic increases by a large factor: the number of
%   hosts (\S\ref{sec:background}).
%   \notepanda{Using this instead of the Overleaf comments, which don't seem to handle returns well. A few things here: (a) we might want to talk about coherence domains or engines rather than cores, given the CXL design; (b) we might want to refer to the slightly more involved CXL coherence mechanism, with the back invalidate, since this makes communication more involved (invalidation is not just core-to-core, but rather core-memory-core now; (c) finally, assuming this is the John Kelm work (Reigel and Cohesion), the goal in that case was somewhat different: combining the performance of accelerator like weak memory models and their performance, with the simplicity of hardware CC, rather than just a concern about scaling. That said, there are ways they describe things that might be useful to us in the paper. But I think the comparison is a bit more involved than what is attempted here.}
% For shared disaggregated memory, a coherence protocol over a remote interconnect exacerbates latency and coherence traffic, as the distance is greater and more CPU caches can contend for cache lines .\noteamaro{I modified the last 2/3rds of this paragraph to try to address Onur's concern (they are on overleaf comments). Please check.}
%In fact, cache coherence is expensive even
%  within a host;
%  %, as the number of cores increases;
%  this cost increases further with disaggregated
%  memory as both system size and memory latency increase
%  (\S\ref{sec:background}).

\noteion{The argument of cache coherence is too expensive for multi\-core is expensive -> multi\-node is obvious. But natural question is what are we going to lose if we drop cache coherence in disaggregated memory?}
\notejae{I gave him some current examples of disaggregated memory use cases and they need minimal coordination across the nodes. He thinks we should put this earlier in the paper to address the question (what will happen if we lose cache coherence). Also as Ion is not as familiar as us in disaggregated memory, he wanted to see the real/practical use cases of disaggregated memory and consequence of no cache coherence }
In this paper, we find that cache coherence
  is too costly when
  disaggregated memory scales to a rack of 20--80 hosts.  
Instead, we propose a different model of coherence
  called \emph{\weakcoherence}, designed
  to leverage the existing hardware-based coherence protocol within
%\noteonur{"hardware-based" coherence protocol}
  each node without paying for the price of coherence
  across nodes.
More precisely, with \weakcoherence, accesses to disaggregated memory remain coherent between caches in the same node but may lose coherence across caches in different nodes\footnote{A node refers to a host or a NUMA domain within a host.} (\S\ref{sec:newcoherence}).
%with one or two CPU sockets,
%  or an individual CPU socket of a host with a large
%  number of sockets\noteamaro{This sentence is off, it seems the last word should have been 'cores'? The limitation to two sockets is also strange. How about we say a node refers to 'a single host or a single NUMA-domain'? I don't think we should be concerned about the case a node has two CXL ports}.
%\notepanda{This next sentence seems repetitive (we explained twice above). Maybe drop?}In summary, coherence holds locally but not remotely.
To function correctly under \weakcoherence, software must
  deliberately manage ownership of data, but
  this can be done in a scalable manner
  at the granularity of nodes rather than
  individual caches within a node (\S\ref{sec:proposal}).
%  (leveraging the local guarantee).
%\notepanda{For previous sentence, I wonder if we want to be a bit clearer that our expectation with \weakcoherence is that software is core to maintaining correctness. This mostly involves changing `Software operates with' to something like `\weakcoherence architectures depend on software to maintain correctness:\ldots'}

Programming with \weakcoherence 
  is more challenging
  than with traditional coherence due to two factors.
First, \weakcoherence
  introduces an unfamiliar programming model where
  memory accesses can have anomalies
  and traditional consistency guarantees are broken (\S\ref{sec:anomalies}). 
Second, ensuring consistency of data shared across nodes
  falls upon the software, requiring explicit management of caches through mechanisms like flushing or
  bypassing caches. This adds complexity and 
  impacts performance if not done carefully.

To address these challenges, we propose building
  application libraries that provide high-level
  abstractions (\eg{} data structures, coordination
  primitives, shared logs, transactions, etc.)
  with strong consistency despite running on 
  hardware with \weakcoherence (\S\ref{sec:proposal}).
Application developers can then use these libraries
  without having to worry about the anomalies of
  \weakcoherence.
%\notemarcos{What is in philip\_cxl related to this?
%  (this was in outline)} \noteamaro{\cite{philip_cxl} says one major blocker for cxl adoption is resulting software complexity that developers need to handle. I think you are already addressing this because of the preceding paragraph.}
We argue that providing consistency for the high-level
  abstractions
  is cheaper than providing full coherence
  for shared disaggregated memory for two reasons.
Firstly, achieving consistency does not
  require every memory access to be cache coherent. Instead, consistency can be provided at a larger granularity; \eg{} at the transaction level in a transaction runtime.
Additionally, high-level libraries have more
  semantic information about applications than
  a stream of loads and stores observed at the
  memory level.
For example, libraries can flush caches only
  at specific points
  (\eg{} when a transaction commits or after
  batching multiple writes), or may bypass
  caches altogether for critical modifications
  using non-temporal writes.

In summary, when scaling shared disaggregated memory,
  we cannot afford the cost of full hardware-based cache coherence.
Therefore, we propose \weakcoherence as a way to
  avoid the overheads of cache coherence on disaggregated memory while
  leveraging the existing coherence mechanism within
  each node.
We further propose building application libraries with high-level abstractions that provide strong consistency guarantees for those abstractions, despite running with \weakcoherence.
In the rest of this paper, we further detail
  this argument, the new coherence model, and
  how it can be used to build strongly consistent
  libraries.

%\notepanda{Repeating a commented out comment above: nothing so far has said that scaling disaggregated shared memory is important. So one might ask, why not just use message passing instead, if scaling is a problem. Maybe we explain this later, or want to, but if so a forward pointer would be good to add.}

\endinput 

\hrule

\begin{outline}
\0  Computer systems today are cache-coherent
    \1 Each CPU caches data locally
    \1 coherence: CPUs never sees stale data in its cache
    \2  stale = old copy not updated after another CPU writes
    \1 with coherence, application threads can use synchronization instructions (atomics, barriers, etc) to share data consistently
    \1 Figure showing two CPUs and their local caches. Line 1) "coherence protocol" between caches; Line 2) "memory access" between caches and memory

\0 Coherence is expensive
    \1 Requires a cache coherence protocol
        \2 Cache lines can be in a number of states (e.g., MESI)
    \1 Need to track states: two main mechanisms:
        \2 Snooping does not scale (too much noise, bandwidth overhead)
        \2 Directory-based adds latency and creates bottlenecks

\0 CXL memory disaggregation
    \1 New hardware allows external shared memory
    \1 Coherence is even harder in shared disaggregated memory
        \2 Much larger systems (memory is attached to many hosts, each with many CPUs)
        \2 Communication between hosts is slower => coherence protocols are also slower
    \1 Position: we will need to live with incoherence
    \1 CXL in fact allows incoherence

\0 The problems with memory incoherence
    \1 Unwieldy programming model
    \1 Software needs to coordinate memory accesses. Could result in
       \2 Complex protocols
       \2 Lower performance than coherence protocols: software communication is slower

\0 Proposal
    \1 Build primitives that ensure consistent shared data atop a memory-incoherent system
        \2 we don't expect developers have to reason about memory incoherence, instead, they should leverage primitives that abstract away the complexity~\cite{philip_cxl}
    \1 Consistency vs coherence: consistency reflects higher-level semantics (e.g., data structures)
    \1 Consistency can be cheaper: not every memory access needs to be coherent to ensure consistency
    \1 What primitives to provide?
    \1 low-level, or core: one-to-one message queue
        \2 with a message queue, we can exchange information between processes across shared disag. memory.
    \1 medium-level (internally these use 1-to-1 queues):
      \2 a monitor informs a process a condition has been met. the process that updates the value runs the monitor logic to determine if anyone should be notified.
      \2 many to many message queues (pubsub): allows processes to exchange events/messages with high perf.
      \2 key-value store: exchange data with high perf. and low memory duplication.
      \2 shared logs
      \2 transactions
    \1 \noteamaro{I changed this point a bit. I think that providing abstractions is better than low level primitives (\eg{} a key-value store that makes sure keys and values are consistent, rather than providing a lock for developers to write a shared table where we can share data.). Also, I believe we can build all the other primitives given a one-to-one message queue, check.}
\end{outline}







==> hotnets24/S2background.tex <==
\section{Background and Motivation}
\label{sec:background}


\subsection{Shared Disaggregated Memory}
%\noteamaro{I think we need to say something about message passing and shared memory, before we talk about shared disaggregated memory. Based in meeting: we are not clearing the debate here, we are going to shared memory}

%\notepanda{Maybe this is answering my question from above, but it worries me a bit. As I see it, the para below says it helps in three ways: (a) overcomes memory wall; (b) eliminates memory strading; and (c) removes RPC cost. My worry for (c) is we also add some tax, so there is a question of how they compare. (a) and (b) seem a bit further away from our point: both can be fixed without sharing? Maybe we should sharpen this a bit to our setting, in particular focusing on \emph{sharing}.}
In this paper, we focus on distributed systems that use shared disaggregated memory\footnote{In this paper,
  the term (shared) disaggregated memory refers to
  memory addressable by 
  load and store instructions, as opposed to mechanisms such as
  RDMA or page faults (which are less concerned
  about cache coherence).} for communication. There is a longstanding debate about whether message passing or shared memory is the best way to build scalable systems. We do not take a position on this debate; instead, we note that existing hardware has made it feasible to build shared memory systems using off-the shelf parts. At the same time, the increasing memory demands of modern workloads, and a slowdown in the
  improvement of local memory capacity has led to increased adoption of disaggregated memory systems. These systems allow multiple servers to combine their compute power to
  process data placed on large pools of shared memory, and could 
 provide the computational capacity of an expensive scale-up supercomputer~\cite{nvidia_dgx_gh200} using commodity hardware.
While early disaggregated memory deployments have 8--16 sockets~\cite{pond}, we envision future rack scale
system with 20--80 servers using CXL v3 switches~\cite{cxl}.
%  of TB.
  
%Modern distributed workloads must process increasing amounts of
%  data in memory, which requires scaling both the memory and
%  processing capacity of a system.
%To provide this scale, 
%  disaggregated shared memory\footnote{In this paper,
%  the term disaggregated (shared) memory refers to
%  memory that is addressable by processor
%  loads and stores, as opposed to mechanisms such as
%  RDMA or page faults (which are less concerned
%  about cache coherence).}
%  provides a compelling solution
%  whereby multiple servers combine their compute power to
%  process data placed on large pools of shared memory.
%For example, deployed on a rack, a disaggregated memory system
%  may have 20--80 servers with a shared memory of 100s or 1000s
%  of TB.
%This provides the computational capacity of an expensive scale-up supercomputer~\cite{nvidia_recent_sc}
%    while leveraging commodity hardware.
% Unfortunately, memory capacity is limited (a few TB 
%   per node at most), memory is expensive (it constitutes more than 50\% of the rack cost~\cite{}),
%   and data exchange is inefficient (e.g., due to
%   network RPC overheads and associated data center tax~\cite{barroso}).
% Disaggregated memory addresses these problems:
%   it increases memory capacity beyond what fits in a
%   node, it improves memory utilization through
%   pooling~\cite{pooling}, and it enables efficient
%   exchange of data through sharing~\cite{shared-disagg-memory}.

Disaggregated memory is not a new concept~\cite{LCMRRW2009}
  but recently, several technologies have emerged
  to support it, including CC\-IX~\cite{ccix}, Gen-Z~\cite{genz},
  OpenCAPI~\cite{opencapi}, and more recently CXL~\cite{cxl},
  which has become an industry standard with broad
  support from hardware vendors.
Conventional wisdom says that shared memory should be cache coherent~\cite{MHS2012},
and the latest CXL v3 specification supports it.
%toprovide cache coherence once hardware is available.
% Cache coherence enables hardware-supported caching of remote data while maintaining traditional memory semantics, allowing access through simple \texttt{\small LD}/\texttt{\small ST} CPU instructions.
  
%In fact, all modern processors provide cache coherence
%  and likewise for the aforementioned disaggregated memory technologies.

% The landscape of high-performance computing increasingly relies on specialized interconnect technologies to alleviate data bottlenecks.
% Among these, several prominent contenders have emerged, each with unique strengths and areas of focus.
% CXL (Compute Express Link), driven by Intel and widely adopted, excels in CPU-accelerator communication, offering various coherency levels for optimized data sharing.
% CCIX (Cache Coherent Interconnect for Accelerators), while facing slower adoption, offers similar capabilities but with a focus on heterogeneous systems.
% Gen-Z, recently merged with the CXL Consortium, provides a broader memory-semantic fabric suitable for disaggregated architectures, emphasizing high bandwidth and flexibility.
% OpenCAPI, championed by IBM and now open-sourced, targets memory and accelerator attachment with a focus on open standards.
% NVIDIA's NVLink, meanwhile, prioritizes high-speed GPU-to-GPU communication within its ecosystem.
% Similarly, AMD's Infinity Fabric caters to high-bandwidth, low-latency connections within its CPUs and GPUs.
% While CXL currently dominates the CPU-accelerator landscape, the evolving demands of data-centric workloads and the push for open, composable systems ensure a dynamic future where these technologies may coexist and cooperate to unlock the next level of computing performance.
% However, all these technologies besides NVLINK and Gen-Z inherently bring cache coherency in their protocol.

% Recently, the Compute eXpress Link (CXL) consortium
%   introduced a mechanism to attach CPU-addressable
%   memory to a host
%   through the PCIe bus, which enables memory
%   disaggregation, including pooling and sharing.
%Reminder: Philip~\cite{philip_cxl} said pooled memory has limited utility, but we go beyond pooled memory since we want to share it.}


\subsection{Cache Coherence and Its Cost}
\label{sec:costcoherence}

Hardware-based cache coherence is prevalent in
  modern 
  multi-core processors.
Typically, each core has individual small caches (\eg{} L1 and L2), and the cores within a processor package share a larger cache (\eg{} L3).
As many cores may access the same memory locations, a location can be simultaneously present in multiple caches.
Cache coherence ensures that
  different cores are provided a consistent view of a
  cache line.
  %(usually with a size of 64-bytes).
%\notemarcos{Panda, is this example better?}\notepanda{Is better, can we perhaps say cached at multiple cores, instead of in multiple caches? My worry with multiple caches is that it includes cases where it is in L1, L2, and L3.}
For example, if a cache line present in multiple caches gets modified by a core, cache coherence ensures that the cache lines are either invalidated or updated.
  % core modifies a cache line in its cache,\notepanda{Note, this example might be too simplistic. If the cache line is already modified or exclusive, no invalidation is needed.}
  % cache coherence invalidates the cache line for the same location in
  % other caches.\notepanda{Can we perhaps remove the multi-layer bit, my worry otherwise is that it gets really complicated. Some processors have WT L1 caches (AMD Bulldozer for instance), and so modifies go through. Generally, I find mixing multilevel and invalidation complicated, because it depends on things like are lower levels inclusive or not, etc.}
% for example
% Coherence combined with the use of the proper synchronization
%   primitives (atomics, fences, etc) ensure that
%   application threads can share data consistently:
%   if one thread writes to a location, another thread
%   can observe the written data.

Cache coherence is implemented through a protocol
that involves CPUs and caches.
This protocol scales poorly because it must
  coordinate the execution of operations across all participant caches, creating a communication bottleneck.
%(e.g., it involves
%  quadratic communication between all pairs of caches, or it
%  creates contention on a common bus, or it creates a bottleneck
%  at a directory entry).
For example, in the MESI coherence protocol~\cite{mesi}, each cache
  line can be in one of four states (Modified, Exclusive, Shared, Invalid), and the caches coordinate to ensure that lines for the same location in different caches are in compatible states.
%For example, a cache line in the Exclusive state in a cache
%  must be in the Invalid state in other caches.
Keeping track of cache line states means that caches need to snoop on the bus, creating a point of contention that limits scalability.
Alternatively, systems with a large number of cores, including
  CXL-based disaggregated memory, use directory-based coherence protocols,
  which scale better
  but add complexity and latency to accesses, and their scalability still falters when a cache line is widely shared.

\eat{
  \notepanda{This is a bit disconnected from the previous paragraph, and the next. I am not sure we use this anywhere (maybe later, but see comment there), so I am confused about what we want the reader to get from this paragraph.}
  CXL disaggregated memory falls into the latter category and uses a directory-based scheme:
  a \emph{home agent} in the disaggregated memory controller
  keeps a directory (the \emph{snoop filter})
  to track which nodes contain a given location;
  the home agent sends \emph{back-invalidate} messages to the nodes
  to invalidate cache entries as necessary.
  %  This mechanism is similar to the one used between CPU sockets with a key
  %  difference\notepanda{This is not that different, ARM does the same thing \url{https://developer.arm.com/documentation/100023/0100/functional-description/operation/snoop-filter}, I would be surprised if Intel or AMD never shipped a chip that did this. Snoop filter size presents a trade-off.}:
  The snoop filter  
  may not have space for all cache lines, 
  so it may need to evict entries (by invalidating
  cache lines in the relevant nodes) or track some entries at a
  coarser granularity (by combining multiple cache lines into a single
  entry).
%This difference saves memory for the snoop filter but increases
%  memory traffic.
}

\begin{figure}[]
    \centering
    \includegraphics[width=0.9\columnwidth,trim={20pt 10pt 20pt 10pt},clip]{figures/AMD Topology.pdf}
    \caption{Evaluation platform. A two-socket AMD EPYC 7754 server,
    with 128 cores per socket. Each socket has 16 core
    complexes with 8 cores each. A core complex corresponds to
    a \emph{soft-NUMA domain}: communication latency is smallest between CPUs in the same complex (same soft-NUMA domain), then within the same socket (same NUMA domain), then across sockets (different NUMA domains), as shown by the latency numbers in blue.
    The server runs RedHat Enterprise Linux 9 with the 5.14 kernel.
    }
    \label{fig:hardware}
\end{figure}

% \begin{figure*}[t]
%   \centering
%   \begin{subfigure}[t]{0.32\textwidth} % Adjust width for 3 graphs
%     \includegraphics[width=\textwidth]{figures/extrapolate.pdf}
%     \caption{Overhead of cache coherence as we vary the number of cores.}
%     \label{fig:many_core}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[t]{0.32\textwidth}
%     \includegraphics[width=\textwidth]{figures/differential.pdf}
%     \caption{Derivatives of overhead in~\cref{fig:many_core}.}
%     \label{fig:derivative}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[t]{0.32\textwidth}
%     \includegraphics[width=\textwidth]{figures/softnuma.pdf}
%     \caption{Overhead of cache cache coherence as we vary the number of soft NUMA domains.}
%              %Placing threads across multiple soft NUMA nodes exacerbates the performance degradation, highlighting the impact of physical core location and cache coherence overhead.}
%     \label{fig:softnuma}
%   \end{subfigure}
%   \caption{The cost of the cache coherence protocol as contention and inter-CPU latency increase.}
%   \label{fig:allgraphs}
% \end{figure*}

\begin{figure*}[t]
  \centering
  \begin{subfigure}[t]{0.32\textwidth} % Adjust width for 3 graphs
    \includegraphics[width=\textwidth]{figures/extrapolate.pdf}
    \vspace{-7mm}
    \caption{}
    \label{fig:many_core}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figures/differential.pdf}
    \vspace{-7mm}
    \caption{}
    \label{fig:derivative}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figures/softnuma.pdf}
    \vspace{-7mm}
    \caption{}
             %Placing threads across multiple soft NUMA nodes exacerbates the performance degradation, highlighting the impact of physical core location and cache coherence overhead.}
    \label{fig:softnuma}
  \end{subfigure}
  \caption{(a) Overhead of cache coherence as we vary the number of cores. 
  (b) Derivatives of overhead in~\cref{fig:many_core}.
  (c) Overhead of cache cache coherence as we vary the number of soft NUMA domains.}
  
  \label{fig:allgraphs}
\end{figure*}


In the remainder of this subsection, we present experiments conducted to understand the cost of cache coherence using the hardware in \cref{fig:hardware}. As the figure shows, the communication between cores exhibits different latencies depending on whether the cores are in the same soft-NUMA domain, the same NUMA domain, or different NUMA domains.
This setup allows us to study the effect of communication latency on coherence overhead.
%
%
% to demonstrate our two observations in
%\S\ref{sec:intro}: 1) the performance impact of modifying a memory location as
%we increase the number of cores. 2) the performance impact of increasing
%communication latency for the cache coherence protocol. For these experiments,
%\noteamaro{a sentence or two about why we are showing hard-numa and soft-numa cost}
%when a cache coherence relative to the
%number of cores and physical distance on a 256-core AMD EPYC 7754 machine.

In the first experiment, we compare two scenarios.
In scenario 1, a number of threads run a loop that atomically increments a single common global variable, thereby producing significant coherence traffic.
Each thread is pinned to a fixed and dedicated set of cores.
Scenario 2 represents a non-cache coherent system.
Since our server is cache coherent, we mimic the behavior of incoherence by having each thread atomically increment a different local variable.
%rather than a common variable.
In both scenarios, we measure the rate of increment operations.
We calculate the \emph{coherence overhead} as the
  ratio between the non-cache coherent rate to
  the cache coherent rate, which represents the multiplicative slowdown
  caused by coherence.

The 'Empirical Single Node' line in \cref{fig:many_core} plots the measured coherence overhead as the number of cores increases.
The overhead increases nearly linearly with the number of cores, reaching 244 at 256 cores.
%At 256 cores, cache coherence produces a 244$\times$ slowdown.
%for cache coherence over no coherence.
%
To further understand these results,
\cref{fig:derivative} shows the slope (derivative) of the
  coherence overhead curve in \cref{fig:many_core}, smoothed out by a Savitzky-Golay filter~\cite{filter}.
For the first 128 cores, the slope
  is smaller (${\approx}0.9$) as these cores
  are within the same NUMA domain.
The slope then increases to ${\approx}1.2$, corresponding
  to a higher overhead per additional core.
This increase happens because after 128 cores, we allocate
  new cores from the second NUMA domain, so the
  coherence protocol experiences higher
  communication latency, increasing the
  coherence overhead.
%
%
% We also observe that communication latency for the coherence protocol impacts 
% performance.
% The first 128 cores are in the same NUMA domain---hence are subject to a smaller CPU-to-CPU communication latency---thus resulting in a smaller slope (around 1) compared with the right part of the figure (with a slope around 1.25).
% We see that the higher communication latency increases the cost of adding more cores.
%
% \notejae{This paragraph is to tell how the performance aligns with cache comm cost}
% The empirical line from~\cref{fig:many_core} has small spikes every 8 cores where it crosses the soft-NUMA boundary and a bigger spike at 128, the NUMA boundary.
% The spikes are in accordance with the cache communication cost of~\cref{fig:hardware} (1:4.13:7.16).
% The average performance degradation within intra-soft-NUMA is 0.66.
% Whenever a thread is added to a new soft NUMA, the average performance degradation of adding new soft numa is 2.81 (causing little spike at every 8 core interval).
% At number of threads is 129 where it crosses the hard NUMA boundary the degradation is 5 making the spike ratio (1:4.27:7.57) which follows the cache communication costs ratio (1:4.13:7.16).
%\notemarcos{Jae, pls chk next to end of para. However: I think
%  this is very hard to digest, maybe nuke this? I believe
%  the argument above about Fig 2b is very similar, albeit
 % with less numeric justification}
 % \notejae{I agree, commented out}
\eat{
In fact, we find that the delta of the
  coherence overhead in~\cref{fig:many_core} as we add 
  a core closely
  tracks the communication latency incurred 
  by the core being added.
}

\if0
More precisely, the increase in the overhead is
  ${\approx}0.66$, ${\approx}2.81$, or ${\approx}5.0$ whenever we add
  a core in the same soft NUMA domain,
  a new soft NUMA domain, or a new NUMA domain,
  respectively.
These proportions $0.66 : 2.81 : 5.0$ closely track the
  proportions $25.8\t{ns} : 106.6\t{ns} : 184.9$\t{ns} of the
  communication latencies within a soft NUMA domain,
  across soft NUMA domains, and across NUMA domains
  in~\cref{fig:hardware}.
\fi



%
%
% Similarly the slope of the graph from thread number 1 to 128 (intra-soft-NUMA only) is 0.87 and thread number 129 to 256 (inter-hard-NUMA) is 1.19 making 1:1.36.
% This roughly matches inter-soft-NUMA:inter-hard-NUMA (1:1.73) cache communication ratio.
% We estimated the slope of multi-node cache coherence to follow slope ratio.
% Latencies of 200, 400, 800 are 1.87, 3.75, and 7.5 times slower than inter-soft-NUMA communication 106.6.
% Thus, the slope should be 1.87, 3.75, and 7.5 times steeper than inter-soft-NUMA only.
% The cache coherence cost deteriorates the performance dramatically, simply having 7.5x slower latency can degrade the performance 1000$\times$.


%We also see smaller oscillations in the slope (one
%  oscillation for every 8 cores), which occurs because there is
%  a small spike every time we involve another core complex
%  (soft NUMA) to the execution.

We next study the effect of communication latency on
  coherence overhead using the soft-NUMA properties of our platform.
From~\cref{fig:hardware}, the latency between
  two cores in the same soft-NUMA domain
  is smaller than across domains.
So we repeat the previous experiment with only 8 cores, but we vary the 
   number of soft-NUMA domains (within a socket)
   from which these cores are chosen.
%\cref{fig:softnuma} shows the results.
As shown by \cref{fig:softnuma}, performance declines as we add more soft-NUMA domains.
%To further elucidate the effects of physical core location on cache coherence, we replicated the experiment from \cref{fig:many_core} using different soft NUMA configurations. 
%Our testbed consists of 16 soft NUMA within the same CPU, each with 8 cores.\noteamaro{we should explain what we mean by soft NUMA}
%Eight threads were run on various soft NUMA placements.
%\cref{fig:softnuma} presents the results from various soft NUMA placements,  
%
When all threads are in the same soft NUMA domain, the
  coherence overhead is 4.3.
Crossing soft-NUMA boundaries increases the overhead to 7.3 with 2 soft-NUMA domains, peaking at 11 when using 8 soft-NUMA domains (\ie{} one core from each).
If we place threads across NUMA domains (not shown) rather than
  soft-NUMA domains, the coherence overhead is 13.5. 
Overall, we see that communication latency significantly affects 
  coherence overheads.

%\notemarcos{Jae, pls chk next}
Hardware with shared disaggregated memory
is not yet commercially
available, so we estimate its coherence overhead as
 follows.
We consider three values for the communication
  between nodes using disaggregated memory:
  200, 400, or 800ns.
This corresponds to a best-case and worst-case
  estimate of disaggregated memory performance
  reported in a recent study~\cite{pond}.
To find the coherence overhead for these
  latencies, we extrapolate our empirical
  measurements of overhead for a single node
  as a function of the communication latency
  incurred for that node both
  within and across NUMA domains.
Through interpolation, we find a
  near linear relation between the
  derivative of the coherence overhead and
  the communication latency\footnote{Specifically,
   the slope of the graph from cores 1 to 128 (within a NUMA domain) is 0.87, while the slope from cores 129 to 256 (across NUMA) is 1.19.
   The proportion 0:87 : 1.19
   nearly matches the proportion 184.9ns : 106.6ns of the communication
   latency across and within NUMA domains 
   in~\cref{fig:hardware}.}.
Thus, for a communication latency of 200, 400, or 800ns
  under disaggregated memory, the
  derivative of the coherence overhead should be
  2.2, 4.5, or 8.9, respectively.
  %1.87, 3.75, and 7.5 times steeper than intra-soft-NUMA only.
  %1.19 * 1.87 = 2.23
  %1.19 * 3.75 = 4.46
  %1.19 * 7.5  = 8.9
This estimate is shown as the Est Multi Node lines in
  \cref{fig:many_core}.
We see that cache coherence
  significantly  affects performance: with an 800ns
  latency, the coherence overhead exceeds
  1000 with 384 cores.



These experiments illustrate why cache coherence scalability is problematic for disaggregated memory. Two factors combine to cause costs to balloon:
the high number of cores, which increases coherence overheads linearly, and the larger communication latency, which proportionally increases its derivative.

% These experiments illustrate
% that the cost of cache coherence is directly impacted by both the number of cores involved and the communication latency over which the cache coherent protocol runs.
% The significant performance overhead demonstrated in our experiments strongly suggests that maintaining cache coherency in modern memory interconnects like CXL may not be advisable.
% \notepanda{I think we might want to tie these results closer to the two factors we mentioned in the Introduction. Currently it is a bit weakly connected?}

\if 0
\begin{outline}
\0 Show non-scalability of coherence with microbenchmarks {\bf the list below is stale}
    \1 Proposal 1: scalability of fetch-and-add (simplest atomic op)
      \2 vary number of threads until the largest number we can
      \2 place memory on a NUMA node that is remote to the threads
      \2 1) local memory; 2) remote NUMA; 3) CXL.
      \2 we can also measure inter-NUMA bandwidth while experiment runs with intel's PCM tool
    \1 Proposal 2
      \2 same setup as 1, but implement a SOTA scalable lock instead of just using FAA
      \2 dpdk has one; intel tbb has another one
    
\end{outline}
\fi

\section{\WeakCoherence}

%\subsection{Definition}
\label{sec:newcoherence}

We define \weakcoherence following two common practices in coherence definitions~\cite{SWD2011}.
First, coherence is defined separately from the memory model,
  by considering the order of operations issued by processors to the cache
  controller rather than the program order.
  %(which may allow instruction re-ordering and other
  %quirks)---thus, the coherence definitions are with respect to the
  %order of operations issued by the processors
  %to the cache or memory controller, rather than
  %the program order.
% Second, the definitions cover only load and store operations
%   not read-modify-write operations (compare-and-swap, fetch-and-add, etc).
Second, coherence is defined for a single fixed memory location rather than the entirety of memory.
%
We start with the standard 
  cache coherence definition~\cite{SWD2011},
  where memory operations are 
  $\t{write}_p(v)$ and $\t{read}_p(v)$, 
  representing a store and load of $v$ 
  by processor $p$ at a fixed memory location.

\begin{definition}
\label{def:coherence}
  A memory system satisfies \emph{cache coherence} if, for every execution and each memory location $\ell$, there is a total order $\mathcal{O}$ of operations on $\ell$ in the execution, such that:

  \begin{enumerate}
  \item $\mathcal{O}$ is consistent with the order of operations on $\ell$ issued by each processor $p$.%\notepanda{Order of operations makes this sound like we are assuming SeqCst? Maybe issued is the problem?}

  \item In $\mathcal{O}$, a read $r$ returns the value of the last write that precedes $r$.
  \end{enumerate}
\end{definition}

\noindent For convenience, we assume that the execution
starts with $\t{write}_{p_0}(v_0)$, representing
the initialization value $v_0$ of $\ell$ by a
hypothetical processor $p_0$.
%
Thus, Definition~\ref{def:coherence} states that operations on a memory location can be serialized,
such that a read always
returns the value of the latest write.
%(where the
%serialization may differ from location to location).

For weaker forms of coherence, we extend processor operations
  to include $\t{flush}_p$, 
  representing a flush of the cache of processor $p$ to memory.
%
  % \noteamaro{Can we unify the definition of flush to always flush from a shared cache? I believe this modified condition doesn't require us to make the flush here only apply to processor p's cache. This would allow us to have a single definition of flush}
  % \notemarcos{if we use a single shared cache in this definition, we get full coherence because caches cannot diverge}
%  
We now define a system with
  a weak form of coherence where processors
  can explicitly flush their caches.
This definition is obtained by modifying condition (2) in Definition~\ref{def:coherence} as follows:

{\it
  \begin{enumerate}
  \item[(2)] In $\mathcal{O}$, a read $r$ returns a
  value picked as follows:

  \begin{enumerate}
      \item If the last operation by $p$ preceding $r$ is $\t{write}_p(v)$ or $\t{read}_p(v)$, pick value $v$.

      \item If the last operation by $p$ preceding $r$ is
      $\t{flush}_p$,
%
\eat{
      $r$ returns the value $v$ from the last $\t{write}_q(v)$
      preceding the most recent $\t{flush}_q$ by any processor $q$.\noteamaro{check--original eaten below}
      \notemarcos{the notion of ``most recent'' isn't
                 clear.}
}
      find the process $q$ with the
      last $\t{flush}_q$ preceding $r$
      %(this could be $q=p$)
      and pick the value $v$ from the
      last $\t{write}_q(v)$ preceding the $\t{flush}_q$.

  \end{enumerate}

  \end{enumerate}
}

Intuitively, this condition says that a read should
 return either the value in the local cache or the
last value that was flushed to memory, depending on whether the reading processor recently flushed its cache.
For convenience, we assume the execution
starts with $\t{write}_{p_0}(v_0)$ followed by $\t{flush}_p$ for every processor $p$.
%\notevincent{the initialization probably needs updating here (fake flush)?}

\eat{
  We next give a definition of \weakcoherence
  where
  all flushes are explicitly issued by the
  program (no cache eviction by the system).
  We obtain this definition by replacing condition (2) of Definition~\ref{def:coherence} with the following:

  {\it
  \begin{enumerate}
  \item[(2)] In $\mathcal{O}$, a read $r$ returns one of the following:

  \begin{enumerate}
      \item If the last operation by some process $p'\in\t{node}(p)$ preceding $r$ is $\t{write}_{p'}(v)$ or $\t{read}_{p'}(v)$, pick the value $v$.

      \item If the last operation by some process $p' \in \t{node}(p)$ preceding $r$ is
      $\t{flush}_{p'}$, find the process $q$ with the
      last $\t{flush}_q$ preceding $r$ and pick the value $v$ from the
      last $\t{write}_{q'}(v)$ preceding the $\t{flush}_q$ with $q'\in\t{node}(q)$.
  \end{enumerate}

  \end{enumerate}
}
}

We now 
  define \weakcoherence
  by modifying the previous definition in two ways.
First, we extend the cache to be shared by all the processors in a node,
  where the intended behavior of a $\t{flush}_p$ operation is to flush this shared cache.
%\noteamaro{should we explicitly say this was not true before?}
%MKA: done, we now say earlier that flush_p represents a flush
%of the cache of processor p.
Second, we allow the total order $\mathcal{O}$
  to include additional flush operations not
  present in the execution,
  representing cache evictions by the hardware.
  %\noteamaro{what system?}.

\begin{definition}
\label{def:weakcoherence}
  A memory system satisfies \emph{\weakcoherence} if, for every execution
  and each memory location $\ell$, there is   
  a total order $\mathcal{O}$ that includes all
  operations on $\ell$ in the execution and
  possibly additional $\t{flush}$ operations, such that:

  \begin{enumerate}
  \item $\mathcal{O}$ is consistent with the
      order of operations on $\ell$ issued by each processor $p$.

  \item In $\mathcal{O}$, a read $r$ returns a value picked as follows:

  \begin{enumerate}
      \item If the last operation by any processor $p'\in\t{node}(p)$ preceding $r$ is $\t{write}_{p'}(v)$ or $\t{read}_{p'}(v)$, pick $v$.

      \item If the last operation by any processor $p' \in \t{node}(p)$ preceding $r$ is
      $\t{flush}_{p'}$,
\eat{
      then $r$ returns the value $v$ from the last $\t{write}_{q'}(v)$ preceding the most recent $\t{flush}_q'$ by any processor $q'$, where $q' \in \t{node}(p)$.\noteamaro{check--original eaten}
}
      find the process $q$ with the
      last $\t{flush}_q$ preceding $r$ and pick the value $v$ from the
      last $\t{write}_{q'}(v)$ preceding the $\t{flush}_q$ with $q'\in\t{node}(q)$.
      \eat{\notepanda{This one is a bit strange. What happens when $p, q\in \t{node}(p)$?}
      \notemarcos{$p$ is always in $\t{node}(p)$, so nothing different
      happens. If $q \in \t{node}(p)$, this corresponds to
      the node flushing its cache then reading again from memory.}
      \notepanda{Also what happens if $\t{node}(p)$ does not have the location cached,
      and also does not issue a flush?}
      \notemarcos{Impossible. If the location is not cached, it's
      because a flush happened by the program or due to
      an eviction (that's why $\mathcal{O}$ may include additional
      flush operations)}
      \notepanda{Also, if $\t{node}(p) = \t{node}(q)$, and there is a $\t{write}$ from $\t{node}(q)$ between $\t{flush}_q$ and $r$, do we loose the write?}
      \notemarcos{Impossible. That falls in case (a) above not (b).}}
  \end{enumerate}

  \end{enumerate}
\end{definition}

\noindent Here $\t{node}(p)$ denotes the set with the processors
in the same node as $p$, and
%\noteamaro{Can we add an intuitive summary of def 2?}
$\t{flush}_p$ is an operation by $p$ to
  flush the cache shared by processes
  in $\t{node}(p)$.
Intuitively, Definition~\ref{def:weakcoherence} says that in the serialized order, reads should return either the value in the cache shared by the node, or the last value flushed to memory from one of the shared caches, depending
on whether the reader's shared cache has been flushed.
%by a process in the reader's node.

% The above definition covers only loads and stores but it is
%   easy to extend it to read-modify-write
% operations (\eg compare-and-swap, fetch-and-add).
% \notemarcos{does it make sense for the processor to issue atomic
% operations to the cache or memory controller?}


\heading{Anomalies.}
\label{sec:anomalies}
%
With \weakcoherence, two types of anomalies are possible:
  cross-node stale reads and cross-node broken atomicity.
Cross-node stale reads happen when a read 
  runs at a node different from the one that
  issued the last preceding
  write, causing the read to miss the write and
  return a stale value.
Cross-node broken atomicity happens when
  atomic operations run at two different nodes
  causing them to break their atomic behavior (e.g.,
  two compare-and-swap atomics may succeed when only one was supposed to, or two fetch-and-increment atomics may increment a counter by only one).
These anomalies break existing concurrent data
  structures (e.g., lock-free queues), synchronization primitives
  (e.g., locks, semaphores), and consistency guarantees
  expected by most developers 
  (e.g., release consistency\footnote{Release consistency ensures that modifications done while a lock is held
  become visible to subsequent lock holders.}).

However, with \weakcoherence, such anomalies happen
  only across nodes.
If a read runs on the same
  node as the last preceding write, the read
  returns the correct value.
If two atomic operations run on the
  same node, they preserve their atomic guarantees.
These guarantees are the basis for writing
 application libraries under \weakcoherence (\S\ref{sec:proposal}).

\eat{
\subsection{Implementation}

\notevincent{Since we're over on space, this subsection is a candidate for deletion.}\notepanda{I agree, deleting this if necessary seems fine.}
While a complete design for hardware that provides disaggregated memory with \weakcoherence is well beyond the scope of this paper, here we briefly sketch a possible approach.
The basic idea is that each node runs its internal hardware-based
  coherence protocol as provided in modern processors.
We connect all nodes to the disaggregated memory without additional coherence mechanisms so that when a node flushes its cache to memory, it immediately overwrites the previous contents without coordinating with other
  caches.
Note this implementation is efficient because the coherence traffic is constrained within each node.
% \notevincent{This section is a bit sparse.  Is there anything else we can add? If no time, it's fine to keep as is.}
}

\eat{
We focus on the CXL v3 hardware
  as the leading contender to realize shared
  disaggregated memory.
  \notepanda{Is there a particular thing we do
  in the proposal below that relies on anything from CXLv3?
  Especially given we disable the coherence engine?}
As we explained before, CXL v3 provides (full)
  cache coherence
  through back-invalidate messages from the disaggregated
  memory controller (home agent).
Basically, we obtain a system with \weakcoherence by
  omitting such messages and the snoop filter mechanism that
  supports them.
\notemarcos{Emmanuel: isn't there a way to disable
cache coherence in CXL (e.g., by definition regions
that are not coherent)? How did that work?}\noteamaro{The spec says regions can have software-defined coherence. I think the way it worked in Niagara is, they just exposed the regions to multiple hosts and that's it}
}

\endinput

\begin{outline}
\0 background on cache coherence
    \1 cache coherence enables consistent sharing of data in multicore processors
    \1 from first principles: here's where the scaling problem comes from
    \1 cache coherence vs memory model (TSO)
        \2 cache coherence only talks about caches but not about store buffers
    \1 memory fences

    
\0 CXL cache coherence: Back invalidate snoop
    \1 this will still be bad
    \1 CXL spec allows incoherence: software-managed coherence

\0 what does incoherence means
    \1 lock instructions and atomics don't work
    \1 what is TSO under incoherence
    

\0 (not sure if this should go here) CXL vs NVLink
\end{outline}

==> hotnets24/S3proposal.tex <==
\section{Building Application Libraries with \WeakCoherence}
\label{sec:proposal}

To simplify application development in the context of 
  \weakcoherence,
we propose building application libraries that
  provide high-level abstractions for common shared-memory tasks such as key-value stores,
  shared logs, message queues, etc.
These high-level abstractions will provide strong consistency
  atop \weakcoherence.
For example, the key-value store ensures a \textit{get} from one thread
  always returns the value of the latest \textit{put} for a given key issued from another thread, 
  regardless of node placement of the threads.
This allows developers to use these abstractions without worrying
  about the anomalies of \weakcoherence (\S\ref{sec:anomalies}).
Of course, the primitives in these libraries must be carefully constructed, but this only needs to be done once for all users.

\subsection{Ownership Tailored to Abstraction}
\label{sec:ownership}
To provide consistency despite \weakcoherence, these libraries need to explicitly
 manage the CPU caches by flushing or
 bypassing them.
 %\noteamaro{when reading memory for which they do not have ownership, when releasing ownership or when acquiring ownership}.
For example, if a thread wants to expose new data
in memory to a thread in another node, both threads need to flush their caches:
the first thread flushes to write the new data to memory,
while the second thread flushes to invalidate any old data in its
cache so that a subsequent read finds the new data.
\eat{
 Unlike cache coherence protocols that always transfer dirty cache lines whenever
  it is read or written by another thread\noteamaro{strictly speaking, I think the dirty cache line is not flushed but invalidated}
  \notemarcos{I think it's both flushed and invalidated, but let's discuss},
}
Our approach allows flushing
depending on the semantics and needs of the specific abstraction.
%Importantly, differently from cache coherence protocols---which
%   flush a dirty cache line whenever it is read or written by another
%  thread---the decision of when to flush and what to flush
%  can be based on the semantics and needs of the target high-level abstraction.
For example, threads do not unnecessarily flush intermediate data (e.g., while initializing a structure).
  %the fields of a struct).


Flushing or bypassing CPU caches must be
  done sparingly to minimize performance impact.
This can be achieved by implementing a software-based
  ownership scheme that controls which node can access a chunk
  of shared data in memory---the \emph{owner node} of that shared
  data.
%This scheme determines when a thread should flush or bypass its cache.
% This can be done through an ownership scheme, which
% determines ownership granularity, policy, and mechanisms,
%   based on the semantics of the high-level primitive being implemented.
In particular, threads in the owner node of the shared data need not
  flush their caches when reading or writing the data, and they
  can use atomic instructions for synchronization among themselves.
A flush is required only if the threads wish to expose the chunk of
  shared data to other nodes or relinquish ownership.
The ownership scheme can be highly tailored to the target
  high-level abstraction, by choosing its granularity, policy,
  change mechanism, and change actions, as we now explain.
First, the ownership granularity defines the memory chunk that is treated
  as a unit for ownership purposes; this granularity may vary
  according to the data type.
Second, the ownership policy indicates the conditions that lead to an ownership change.
  For example, in a single-producer single-consumer (SPSC) queue,
  a queue entry changes its ownership dynamically from producer to consumer
  immediately after the producer populates an entry. 
In other applications, ownership may be static (\ie{} never change).
Third, the change mechanism determines how to implement
  ownership change; this requires a consistent way for threads
  to communicate (more on this below).
  % \noteamaro{notifications can be used for ownership change, but they can be used for other things too, I'll fix}
  % \notemarcos{Probably best to fix it in S4.2
  % rather than here}
Finally, the change action indicates what actions must be taken
  when ownership
  changes, such as publishing the ownership granularity to other nodes.

\eat{
To provide consistency in these implementations, we make judicious use of the following techniques:

\begin{itemize}
\item \textbf{Flush caches explicitly and only when necessary.}
With \weakcoherence, if a thread wants to expose new data
in memory to another thread, both threads need to flush their caches:
the first thread flushes to write the new data to memory,
while the second thread flushes to invalidate any old data in its
cache so that a subsequent read finds the new data.
Importantly, differently from cache coherence protocols---which
  will flush a dirty cache line whenever it is read or written by another
  thread---the decision of when to flush and what to flush
  can be based on the semantics and needs of the target high-level abstraction.
For example, it is unnecessary to flush intermediate data
  produced by a thread (e.g., when filling
  fields of a struct).

\item \textbf{Bypass caches altogether.}
Rather than dealing with incoherent caches,
  threads can read\notepanda{Read to what? Register? The write I understand, the read worries me a bit.} and write data in memory
  directly.
This can be advantageous for accesses without
  temporal locality and when a thread
  wishes to transfer data to another
  thread.
Modern processors have instructions
  that facilitate and optimize direct
  memory accesses, such as non-temporal
  loads and stores.
Again, the choice of when to bypass caches is 
  tailored to the semantics of the target high-level abstraction.
% Threads can read and write data in
% memory without any caching. This can be done efficiently if the writing
% thread has a block of data consisting of one or a few cache lines
% that it can write as a whole---such
% an operation can be optimized through special non-temporal
% writes in modern processors.
% Meanwhile, the reading thread can also be optimized by 
% prefetching the block of data.
% \notemarcos{correct? Can we optimize the read in other ways?}
% Again, the choice of when to bypass caches is tailored to
% the semantics of the target high-level abstraction.
\noteamaro{I am concerned with this technique since it is an optimization}
\notemarcos{I rewrote it. I agree the previous text highlighted too much the optimization aspect. Hopefully now, the high level idea (bypass caches since they're not cache coherent) doesn't give the impression of an optimization.}
\notepanda{I found this a bit confusing. I think the point is that when software meets the standard non-temporal requirements (unlikely to see access from the same core) we should use that, but what does that have to do with disaggregation or not. It is true for even multicore processors, no? Are we seeing any benefits from avoiding the cache hierarchy beyond that? Are we imagining cache line sized registers, I guess they are kind of here with AVX512 but then are we really saying people should be using only \texttt{vmovntdqa} for everything?}

\item \textbf{Establish an ownership scheme of who can access shared data in memory and when.}
%This scheme determines when a thread should flush or bypass its cache.
% This can be done through an ownership scheme, which
% determines ownership granularity, policy, and mechanisms,
%   based on the semantics of the high-level primitive being implemented.
A thread that exclusively owns some shared data need not
  flush its cache or bypass the cache, until the ownership changes.
The ownership scheme can be highly tailored to the target
  high-level abstraction, by choosing its granularity, policy,
  change mechanism, and change actions, as we now explain.
The ownership granularity indicates what chunk of memory is be treated
  as a unit for ownership purposes; this granularity may vary
  according to the data type.
The ownership policy indicates what conditions lead to an ownership change:
  for example, in a single-producer single-consumer (SPSC) queue,
  a queue entry changes its ownership from producer to consumer
  after the producer populates the data.
The change mechanism determines how to implement the
  ownership change; this requires a consistent way for threads
  to communicate (more on this below).
Finally, the change action indicates what actions must be taken
  when ownership
  changes (e.g., flush some data to memory).
  \notepanda{The description of this in \url{https://ieeexplore.ieee.org/document/5713322} is quite nice if we want to borrow a similar way.}
\end{itemize}
}

While cache coherence protocols have
  a notion of ownership
  too, they differ from the above notion of ownership 
  %of ownership of shared data 
  because they do not tailor to the target abstraction:
  the granularity is fixed to one or more cache lines,
  the policy is driven by low-level memory accesses,
  the change mechanisms and actions are fixed by the hardware
  (\eg{} the change mechanism might be a MESI protocol message~\cite{mesi},
  and the change action might be to flush the entire cache line).
This one-size-fits-all approach is inefficient for shared disaggregated memory, as we
explained before (\S\ref{sec:costcoherence}).
While we could leverage prior work on
  software coherence protocols (e.g., \cite{swcachecoherence})
%author="John H. Kelm and Daniel R. Johnson and Steven S. Lumetta and Matthew I. Frank and Sanjay J. Patel",
%title="A task-centric memory model for scalable accelerator architectures",
% booktitle="International Conference on Parallel Architectures and Compilation Techniques", 
% pages="77--87",
% month=sep,
% year=2009
  they would need to be further specialized
  to the specific high-level abstraction being implemented.

Eventually, our application libraries will include a large
  variety of useful abstractions, including
  key-value stores,
  shared logs, and transactional stores, as well as lower-level primitives such as monitors and barriers.
We plan to build these abstractions with the approach sketched above.
Next, we give a more detailed explanation of notifications and finish this section with an example of how to apply the approach outlined here to build a
  useful abstraction to share data with \weakcoherence.

\subsection{Notifications}
\label{sec:notific}

We need a notification mechanism for nodes to communicate consistently with each other.
%Implementing such ownership schemes raises the
%question of how threads can communicate consistently in the first place.
For example, a writing thread in one node may need to notify a reading
  thread in another node that a buffer is ready for consumption. 
  Another example is a producer may need to awake a consumer thread in another node to begin consuming data from a queue on shared disaggregated memory. 
How can we implement such a notification when memory is incoherent
  across nodes?
%We believe there are several ways of doing so.
A simple approach is to use message-passing through a network.
We expect all notification messages to be small (\eg{} a few bytes) so these are unlikely to
require high bandwidth or create congestion problems.
As such, we can use techniques such as 
  PFC to provide lossless communication over Ethernet or UDP,
  without concern for PFC storms.
% \notemarcos{We cannot talk about remote interrupts via
% disaggregated memory because SKH disclosed this idea to us and
% they aren't authors.}
% %A second approach is to extend the disaggregated memory
% %  with support for low latency small messages; \eg{} remote interrupts delivered via the disaggregated memory.
% \notemarcos{The approach of using SPSC creates a confusing
%   paper structure. The SPSC is supposed to be an example of
%   a high-level abstraction we can build, not a technique
%   to build high-level abstractions.}
%We believe a better approach, which we detail next, is to use a combination of notifications
%and a Single Producer-Single Consumer queue over incoherent memory.
%The benefit of this hybrid approach is that a single notification can be used to
%communicate many messages over the SPSC queue, since notifications are infrequently required.

%\subsection{Other Primitives}
%\begin{outline}
%\0 Higher level primitives:
%    \1 key-value store: exchange data with high perf. and low memory duplication.
%        \2 how uses SPSC queue
%    \1 many to many message queues (pubsub): allows processes %to exchange events/messages with high perf.
%    \1 shared logs
%    \1 transactions
%    \1 \notepanda{Maybe add more.}
%\end{outline}
% Next, we provide a example of how to use this approach to implement a single-producer single-consumer queue in 
%   disaggregated shared memory,
% where the producer and consumer can be in different nodes.



\subsection{Case Study: MPMC Queue}
\notejae{I think 2 phase locking algorithm would be a better example here. There exists many lock algorithms for non-cache coherent and no atomic operation support processors like Lamport's Bakery algorithm. However, scalability is the biggest disadvantage of these algorithms. We can improve the performance with \weakcoherence by having a node-wise lock as Bakery's algorithm and existing lock within a node.}

We now show how to apply the ideas in
  \S\ref{sec:ownership} and \S\ref{sec:notific}
  more concretely to build a specific
  abstraction:  
  a multi-producer multi-consumer (MPMC) queue.
An MPMC queue allows a set of producers to add
  elements to the queue and a set of consumers to
  remove elements.
We sketch the implementation of an MPMC queue
  that uses
  disaggregated memory with \weakcoherence, where all producers
  run in one node and all consumers run in a different node.
This abstraction can be used for work distribution
  between nodes or as a communication channel across nodes.

We call the node where the producers run the \emph{producer node} and the node where the consumers run the \emph{consumer node}.
%The MPMC queue supports payloads of 63 bytes (one byte less than the cache line size), which can be used to transmit pointers to larger payloads if desired.
The MPMC queue is implemented using a ring buffer in shared disaggregated memory.
%consists of three ring buffers: one in shared disaggregated memory, and two in the private memories of
%  the producer and consumer nodes, respectively.
%The producer and consumer access their private rings without requiring disaggregated memory coherence.
The ring buffer consists of a number of slots, and each slot has one byte for metadata and 63 bytes for the payload (can be a pointer to larger payloads).
The metadata has an \emph{node ownership-bit} indicating what
  node that owns the slot
  (producer or consumer node), and a \emph{used-bit}
  indicating if the slot has been used within the node. 
The node ownership policy is simple: the slot initially
  belongs to the producer node; it changes ownership to the 
  consumer node when the slot is populated by a producer;
  and it changes ownership back to the producer node
  when a consumer receives the payload.
%
%The slot ownership policy is dynamic but simple: only the owner of a slot can access its payload and change its ownership.
%Each slot is owned by one of the hosts at any time, and the ownership bit and payload both fall within an aligned 64-byte block.
A producer publishes its updates by flushing the slot.
%disaggregated memory by with
% one 64-byte write instruction, using its private ring slot as source.

An example of sending payloads from a producer thread $p$ to consumer node $C$ through the MPMC queue is as follows.
%We assume all slots are initially owned by the producer.
\begin{enumerate}
\item Producer thread $p$ selects a slot for the message by compare-and-swap until it finds a clear used-bit.

\item $p$ writes the payload,
sets the node ownership bit to the consumer,
and flushes the slot (a single cacheline).
Finally, if necessary, $p$ sends a notification (\S\ref{sec:notific}) to $C$ with the published slot to the consumer node.
% producer $P$ populates its local slot's payload, sets the node ownership bit to the consumer node,
% % \notepanda{Wait is it targeted consumer node or any consumer? Usually MPMC is any consumer. Did you perhaps mean to a consumer-available bit.}, 
% and then publishes the slot by copying its local slot to the corresponding
% disaggregated memory slot, using a 64-byte write.

\item  Upon receiving the notification, the consumer node wakes up all free cores and provides them with the selected slot. 

\item \label{itm:prev} Each core $c$ tries to clear the slot's used-bit with a compare-and-swap. The succeeded core processes the payload and then moves on to the next step. Failed cores also move on to the next step.
    % \begin{enumerate}
    % \item If the node ownership equals the consumer node, core $c$ tries to clear the used-bit with a compare-and-swap. If the core succeeds, it processes the payload\noteamaro{and then?}. We describe the algorithm followed by the core if it fails to clear the used-bit in~\ref{itm:cont}.
    % % could not clear the used-bit (but the slot was owned by the consumer), then it repeats this process with the next slot. On the other hand, if the core fails because the slot is owned by the producer, it sleeps and waits to receive another notification.
    % %\noteamaro{this last sentence can be confusing relative to what we say in the last paragraph about a consumer being able to discover additional slots}
    % %\notemarcos{indeed, it's contradictory}
    % \item If the core failed because node ownership does not equal consumer, core $c$ retries by flushing its cache line corresponding to the shared disaggregated memory slot, issuing a memory fence, and re-checks the node ownership bit. Consumer $C$ uses a backoff heuristic to save bandwidth. 
    % \end{enumerate}
\item \label{itm:cont} %After a core has processed a slot or moved on because it could not clear the used-bit, it 
Cores try to check if it can process the next slot.
To do so, the core first checks if the next slot is owned by the consumer.
If so, it returns to step~\ref{itm:prev} for the next slot.
On the other hand, if the slot is owned by the producer, the core goes to sleep awaiting the next notification.
\end{enumerate}

Therefore, in our approach, in the best case, a single notification can provide payloads for all cores in the consumer node.
Furthermore, producers in the producer node may continue writing to new owned slots, which consumer cores can discover without additional notifications.
The consumer node sends the producer node a notification when all of its cores go to sleep, telling the producer about the last processed slot.
%The consumer can append replies directly on a slot by overwriting the slot before changing ownership back to producer.
A consumer returns the slot to the producer node by changing the node ownership bit.
A producer can then reuse the slot for another payload.



\endinput


We show how to implement a
  single-producer single-consumer (SPSC) queue that uses
  disaggregated memory with \weakcoherence, where the producer
  and consumer can be in different nodes.
The SPSC queue supports payloads of 63 bytes (one byte less
  than the cache line size), which can be used transmit pointers to larger payloads if desired.

The SPSC queue consists of three ring buffers: one in shared disaggregated memory, and two in the private memories of
  the producer and consumer, respectively.
%The producer and consumer access their private rings without requiring disaggregated memory coherence.
Each ring buffer consists of a number of slots, where each slot
has one byte for metadata and 63 bytes for the payload.
The metadata has one bit indicating the ownership of the slot
  (producer or consumer).
The slot ownership policy is simple: the slot initially
  belongs to the producer; it changes ownership to the consumer
  when the slot is populated by the producer;
  and it changes ownership back to the producer when the consumer
  receives the payload.
%
%The slot ownership policy is dynamic but simple: only the owner of a slot can access its payload and change its ownership.
%Each slot is owned by one of the hosts at any time, and the ownership bit and payload both fall within an aligned 64-byte block.
The producer writes the slot in disaggregated memory with
 one 64-byte write instruction, using its private ring slot as source.

An example of sending a message through the SPSC queue is as follows.
%We assume all slots are initially owned by the producer.
\begin{enumerate}
\item The producer selects a ring buffer slot to use for the message, and sends a remote notification to the consumer with the slot it selected.
\item The producer populates its local slot's payload, sets the ownership bit to consumer, and then publishes the slot using one 64-byte write.
\item Upon receiving the notification with the selected slot, the consumer checks whether it owns the slot:
    \begin{enumerate}
    \item If ownership equals consumer, the consumer reads and processes the payload 
    \item If ownership does not equal consumer, the consumer retries by flushing its cache line corresponding to the shared disaggregated memory slot, issuing a memory fence, and re-checks the ownership bit. The consumer can use a backoff heuristic to save bandwidth. 
    \end{enumerate}
\end{enumerate}

The producer may continue writing to new slots, which the consumer can discover without additional notifications by checking ownership of the next slot with a timeout (similarly to 3 above).
%The consumer can append replies directly on a slot by overwriting the slot before changing ownership back to producer.
The consumer returns the slot to the producer by changing the
  ownership bit.
The producer can then reuse the slot for another payload.
%A producer cannot reuse a slot until ownership changes back to itself, providing back pressure.


%\0 cache coherence protocols rely on per-CL messages across holders of the CL
%    \1 expensive because this happens at granularity of CL (64 bytes) and requires per-cache line messages to coordinate CL holders\notepanda{A reader might wonder if it wouldn't be easier to increase the CL size. I think we should dismiss this earlier, likely in S2.}
%    \1 to improve, we can use these building blocks:\notepanda{Modulo my random comments below, this seems like a good subsection to have here, and something we probably want to highlight in the introduction.} 
%        \2 recognize that not every memory access must be cache-coherent
%        \2 leverage the semantic information from the abstraction to provide consistency at granularities larger than a CL\notepanda{I think we should rephrase this, in some sense we want consistency at the granularity of an object/adt}
%        \2 use memory ownership to determine who can access or modify a block of shared memory\notepanda{Isn't maintaining ownership a bit like maintaining a directory. I think (though I might be wrong) the big difference is we let the applications figure out/manage ownership as they want, rather than maintaining a separate ownership directory.}
%        \2 use remote notifications to signal state changes
%    \1 these core building blocks enable building more general abstractions
    
%\0 core building blocks:
%    \1 memory ownership at different granularities
%    \1 remote notifications to participant processes
%    \1 local memory control: cache line flush, memory fences
%    \1 these core building blocks enable building more general abstractions
    
%\1 Targets payloads of 64 bytes or less, use pointers for larger payloads.
%\1 provides consistent exchange of information across two endpoints (processes in a host), one is the producer and the other is consumer. 
%\1 structure:
%    \2 consists of 3 rings buffers: one is shared in disag memory, and the other 2 are private in producer's and consumer's local memory. producer and consumer access their private rings without the need for disaggregated memory coherence.
%    \2 logically implemented with a ring buffer of 64-byte slots
%    \2 each slot uses 1 byte for metadata leaving 63 for payload. metadata: 1 bit for ownership (producer or consumer), 6 bits for payload size. 
%\1 memory ownership:  
%    \2 policy: only the owner of a slot can access its payload and change its ownership.
%    \2 scope: each slot is owned by one of the hosts at a time and the ownership bit and the payload both fall within a single 64-byte block. therefore, writing to a slot can be done in one shot by using 64-byte writes.
%\1 Example of sending a message:
%       \2 The producer selects a ring buffer slot to use for the message, initially owned by the producer.
%       \2 The producer sends a remote notification to the consumer with the slot it will use for the message.
%       \2 The producer populates its local slot's payload, changes the ownership bit to the consumer in its local ring, and writes the entire slot in one operation to the shared ring using a 64-byte write.
%       \2 The consumer, upon receiving the remote notification with the slot information, checks whether the slot ownership bit indicates it is the consumer. 
%           \3 If ownership equals consumer, the consumer reads and processes the payload.
%           \3 If ownership does not equal consumer, the consumer retries by flushing its cache line corresponding to the slot, issuing a memory fence to ensure memory access order, and rechecking the ownership bit.
%
%%\0 performance of message queue
%%    \1 although one could use a network instead of a message queue, in early experiments the message queue enables high throughput and low latency
%%    \1 in scenarios usually problematic for networks; \eg{} tiny payloads
%%    \1 Intel Xeon Gold 6430. Using 8B payloads:
%%        \2 NUMA RTT: $\approx$1us, and throughput in $\approx$25M op/sec with 1 core
%%        \2 Niagara RTT: 2.96us RTT, 5.2M ops/s.
%%    \1 we have a charts, check with Marcos if we can use them.
%\end{outline}
%
%\notepanda{Why is this better than coherence?}
%\begin{outline}
%\0 Might ask if this construction improves over a SPSC queue built over disaggregated memory coherence.
%    \1 Both require communication and coordination, either to ensure memory coherence or to notify the consumer (or producer) when data (or a slot) is available.
%    \1 So what is different? Number of messages required in the worse case, as we argue next.
%\0 To do so, first need to define the worse case for each, and communication required.
%    \1 Coherent SPSC: a case where the consumer is polling the same cache line that the producer is trying to write to, as might be the case where consumer is polling the head pointer while the consumer is updating it. \fixme{Cite enso and other papers that talk about this phenomenon.}
%        \2 \notepanda{Maybe make this into figure.} WLOG, start with a case where contended cache line is in shared mode so that consumer can read it.
%        \2 At this point, producer invalidates the cache line on the consumer to write. Assume to reduce condition does an increment (so a read and write).
%        \2 Can be interrupted after read by the polling consumer.
%        \2 Result: a pessimistic trace can require an unbounded number of coherence rounds, even to make a single slot visible.
%        \2 While this can be fixed, \eg by adding a backoff to the consumer, the choice of a backoff is crucial, since a bad backoff might exacerbate the situation.
%        \2 Prior work~\cite{enso} shows this is not just a theoretical problem, but one that already occurs when looking at DMA from devices to CPU.
%    \1 Our case: consumer is idle, requiring messaging after a write to the slot.
%        \2 But that is it, there is no consumer behavior, or change in timing that can require additional messages.
%\end{outline}




==> hotnets24/S6related.tex <==
\section{Related Work}
\label{sec:relwork}

\topheading{Disaggregated Memory.} Prior work on disaggregated memory~\cite{aifm, cfm, infiniswap, carbink,scaleNUMA} focuses on expanding the memory available to servers. In this model, a single server owns and has
exclusive access to
each remote memory location. Because the memory is not shared, coherence is not required for correctness. However, nearly all of these systems use a cache (often node-local memory) to reduce latency when accessing remote data, and need to track modifications to update the remote copy when necessary. To do so, prior work uses dirty bits on the page table~\cite{cfm, infiniswap}, or object metadata~\cite{aifm}. Recent work~\cite{calciu2023using} proposes using the node's cache coherence protocol to track modifications at a finer granularity.  However, as data is not shared across machines,
the work addresses a different problem from
ours.

\heading{Distributed Shared Memory, Manycore Processors, and Accelerators.} Cache coherence overheads have been a concern in distributed shared memory systems~\cite{munin, shasta, treadmarks, argo}, and many-core processors and accelerators~\cite{cohesion, conda, sahc}.
In both cases, maintaining coherence is considered important because it simplifies the programming model but raises concerns about scalability. To address this problem, these systems provide mechanisms to tune coherence protocols to the application to reduce coherence traffic.
For instance, Munin~\cite{munin}, a distributed shared memory system, allows applications to specify an object's expected access pattern and, when possible, switches to a protocol specialized to that pattern.
Similarly, Cohesion~\cite{cohesion}, a prototype manycore processor, allows applications to dynamically choose whether coherence for an object is implemented in hardware (using the MESI protocol) or in software (allowing applications to use custom coherence mechanisms, albeit with a performance penalty). Distinct from our proposal, these works require developers to select an appropriate coherence policy. We instead introduce a new coherence
property for disaggregated memory and propose that developers use strongly consistent application libraries that are already designed for the system, reducing development and reasoning burden. 

\heading{Incoherent Memory.} Other works have also focused on implementing coherence in platforms with incoherent memory, such as nodes where memory is shared between processor and accelerator (\eg GPU)~\cite{cosh, popcorn, hare}), between processes running on partitioned global address space~\cite{pegasus}, or on rack-scale, non-cache-coherent shared memory architectures~\cite{BI}. Of these, Bounded Incoherence~\cite{BI} targets the same problem as us, how to scale coherence in rack-scale disaggregated shared memory systems.
However, they differ in the approach: they modify the coherence guarantees so that a processor might read stale data for a bounded amount of time (measured in terms of CPU clock ticks) after another processor has updated the variable.
Delaying updates in this way reduces coherence traffic but makes programming and reasoning about correctness more challenging.
By contrast, we aim to provide developers with familiar, strongly consistent abstractions through our application libraries.

%Hare
%Popcorn
% 
% A different line of work has focused on using software to implement coherence in non-coherent architectures including across heterogeneous accelerators~\cite{BI, hare}, in disaggregated memory systems~\cite{faraboschi2015beyond, argo, scaleNUMA}, and partitioned global address space frameworks employed in HPC clusters~\cite{pegasus}. All of these approaches incorporate optimizations to reduce coherence traffic, a common one being combining writes and delaying invalidations. These optimizations fit into our proposed approach (\S\ref{sec:proposal}) of carefully managing ownership and delaying memory flushes.

\endinput

\notepanda{Jae's text is below, I wanted to reorganize and compare to ours. Feel free to steal or revert.}




\paragraph{Non-coherent memory systems}
have gained attention as the overhead of maintaining traditional coherence across a large number of cores has become increasingly expensive in terms of both performance and energy consumption. 
This has prompted alternative approaches to managing shared memory and maintaining consistency in non-cache-coherent environments, from the language runtime~\cite{chuang2020scaling,libmpnode,jdmm,pegasus} to distributed systems~\cite{faraboschi2015beyond,BI,argo}\notepanda{I would say at the very least, Pegasus is a distributed system too, I also think BI is partly a runtime. So this categoirzation might be strange. Also what is the takeaway?} and operating systems~\cite{cosh,hare}.

Early work in this area includes Munin~\cite{munin}, which introduced the concept of distributed shared memory based on type-specific memory coherence protocols.
This approach allowed for optimizations tailored to specific data types and access patterns.
\notepanda{Shasta did not build on this.}Building on this, Shasta~\cite{shasta} presented a software-only approach for supporting fine-grain shared memory, demonstrating the potential for efficient implementation without hardware support.
\notepanda{So did Munin?}TreadMarks~\cite{treadmarks} further advanced the field by introducing a distributed shared memory system for networks of workstations.
This system implemented lazy release consistency and multiple-writer protocols, significantly reducing communication overhead in distributed environments.

More recent work has focused on addressing the challenges of non-cache-coherent architectures in modern computing environments. 
ARGO~\cite{argo} proposes a distributed approach where nodes can directly request ownership of data from the last writer instead of relying on centralized coherence protocols.
Bounded Incoherence~\cite{BI} introduces a model that allows for controlled levels of incoherence, balancing performance and consistency according to an "incoherence distance", which represents the degree of inconsistency in shared data.
This approach provides a flexible framework for managing the trade-off between consistency and performance.
Another significant contribution is the "Scale-Out NUMA"~\cite{scaleNUMA}, which introduces a scalable, non-uniform memory access model specifically designed for large-scale, distributed systems.
This system effectively handles the challenges of scale by extending NUMA architectures to support scale-out applications. 
It demonstrates how disaggregated memory with \weakcoherence can be managed efficiently, ensuring consistent information sharing across a large and dynamic system without the overhead of full cache coherence, thus optimizing both data access and system scalability.

In the context of PGAS (Partitioned Global Address Space) languages, Pegasus~\cite{pegasus} addresses the challenge of efficient data transfers on non-cache-coherent many-core systems.
This work demonstrates the importance of tailoring memory management strategies to specific programming models and hardware architectures.
Similar to our proposal, \cite{calciu2023using} demonstrated 
a hybrid approach that maintains full cache coherence within local domains (e.g., within a single server) while relaxing coherence across the disaggregated memory fabric can significantly reduce the overhead of maintaining global coherence while still providing strong consistency guarantees for most common access patterns.

These works highlight the need for revisiting memory consistency models and coherence protocols to better suit the characteristics of modern non-cache-coherent systems and workloads.

\if0
\begin{outline}
\0 systems that use remote memory \\
\0 disaggregated memory, and shared disaggregated memory\\
\0 DSM: hardware and software cache coherence
\end{outline}


\notepanda{DSM stuff we should mention}
\begin{outline}
\0 Munin~\cite{munin}
    \1 Type specific coherence
        \2 Coherence tied to expected usage pattern: write-many, synchronization objects (mutex, etc.), migratory object (single accessor at a time), producer consumer objects (similar to our queue), read-mostly object, `general-write' (the other category).
    \1 Loose coherence through a `delayed update queue'
        \2 Collects updates from a thread.
        \2 Releases the eventually: decision on when is based on coherence type.
        \2 The goal is write-combining to increase scaling, so it is rather similar to our goal.
    \1 Was implemented on top of V, and in the old days (Sun workstations connected with ethernet), so the implementation choices don't necessarily map to us.
    \1 Mostly I think summarizing this as a previous approach to building a library that improves coherence might be good?
\0 Shasta~\cite{shasta}
    \1 \notepanda{This is probably the easiest to dismiss, but should be mentioned.}
    \1 Coherence in software.
\0 TreadMarks~\cite{treadmarks}\notepanda{Maybe?}
    \1 Lazy release consistency, so delay flush/release until read.
    \1 Claim is this gives write combining with little additional overhead.
    \1 Might not be that related.
\end{outline}

\notepanda{PGAS?}
Pegasus~\cite{pegasus} is somewhat close to \weakcoherence. The standard PGAS approach is to partition the address space (so single ownership), but Pegasus is worried about what happens with pointers that corss the partition boundary. End up building a software mechanism for fast transfers.

\notepanda{The architecture/Systems papers}
\begin{outline}
\0 Popcorn~\cite{barbalace2015popcorn}: shared objects in heterogenous processors (XeonPHI, etc.).
    \1 Page granularity, uses page replication to give everyone their own copy, and then implements MSI (no E) in software.
\0 
\end{outline}
\fi


==> hotnets24/S7conclusion.tex <==
\section{Conclusion}
\label{sec:concl}

We argued that hardware-based
  cache coherence creates a
  scalability problem for shared disaggregated memory.
We thus proposed a new coherence property,
  \weakcoherence, which 
  provides coherence only within each node.
To simplify application development
  under this weaker coherence, we plan to
  build application libraries that provide
  strong consistency for commonly used
  abstractions.
To build such libraries,
  we proposed using 
  %to handle \weakcoherence
  an ownership scheme tailored to
  the abstraction being implemented.
We gave an example of how to apply this
  idea
  to build a multi-producer multi-consumer
  queue.


